Measurement of the CP asymmetry in $D^+ \to \pi^+ \pi^0$ decays at Belle II

We measure the CP asymmetry in $D^+ \to \pi^+ \pi^0$ decays reconstructed in $e^+ e^-$ collisions at the Belle II experiment using a data set corresponding to an integrated luminosity of 428 fb$^{-1}$. A control sample of $D^+ \to \pi^+ K_{S}$ decays is used to correct for detection and production asymmetries. The result, $A_{CP}(D^+ \to \pi^+\pi^0) =(-1.8 \pm 0.9 \pm 0.1)\%$, where the first uncertainty is statistical and the second systematic, is the most precise determination to date. It agrees with the prediction of CP symmetry from the standard model, and with results of previous measurements.

==> authors/pub084-orcid.tex <==
%%% Paper:    D+ to pi+ pi0
%%% Journal:  PhysRev
%%% Contacts: Y. Jin, A. Di Canto
%%% ====================================================================
%%% Use \input{pub084-orcid} to insert this material into your latex file.
  \author{I.~Adachi\,\orcidlink{0000-0003-2287-0173}} % 2590
% \author{K.~Adamczyk\,\orcidlink{0000-0001-6208-0876}} % 2239
  \author{L.~Aggarwal\,\orcidlink{0000-0002-0909-7537}} % 10083
% \author{P.~Ahlburg\,\orcidlink{0000-0002-9832-7604}} % 2367
  \author{H.~Ahmed\,\orcidlink{0000-0003-3976-7498}} % 11323
% \author{J.~K.~Ahn\,\orcidlink{0000-0002-5795-2243}} % 7423
% \author{Y.~Ahn\,\orcidlink{0000-0001-6820-0576}} % 14363
  \author{H.~Aihara\,\orcidlink{0000-0002-1907-5964}} % 2223
  \author{N.~Akopov\,\orcidlink{0000-0002-4425-2096}} % 9443
  \author{S.~Alghamdi\,\orcidlink{0000-0001-7609-112X}} % 27804
  \author{M.~Alhakami\,\orcidlink{0000-0002-2234-8628}} % 28103
  \author{A.~Aloisio\,\orcidlink{0000-0002-3883-6693}} % 2194
% \author{N.~Althubiti\,\orcidlink{0000-0003-1513-0409}} % 21524
  \author{K.~Amos\,\orcidlink{0000-0003-1757-5620}} % 27583
% \author{L.~Andricek\,\orcidlink{0000-0003-1755-4475}} % 2098
  \author{M.~Angelsmark\,\orcidlink{0000-0003-4745-1020}} % 13963
  \author{N.~Anh~Ky\,\orcidlink{0000-0003-0471-197X}} % 2218
  \author{C.~Antonioli\,\orcidlink{0009-0003-9088-3811}} % 20583
  \author{D.~M.~Asner\,\orcidlink{0000-0002-1586-5790}} % 4684
  \author{H.~Atmacan\,\orcidlink{0000-0003-2435-501X}} % 2538
% \author{V.~Aulchenko\,\orcidlink{0000-0002-5394-4406}} % 8183
% \author{T.~Aushev\,\orcidlink{0000-0002-6347-7055}} % 3747
  \author{V.~Aushev\,\orcidlink{0000-0002-8588-5308}} % 2155
  \author{M.~Aversano\,\orcidlink{0000-0001-9980-0953}} % 7363
  \author{R.~Ayad\,\orcidlink{0000-0003-3466-9290}} % 3766
% \author{T.~Aziz\,\orcidlink{-}} % 3523
  \author{V.~Babu\,\orcidlink{0000-0003-0419-6912}} % 5623
% \author{S.~Bacher\,\orcidlink{0000-0002-2656-2330}} % 2258
  \author{H.~Bae\,\orcidlink{0000-0003-1393-8631}} % 10863
  \author{N.~K.~Baghel\,\orcidlink{0009-0008-7806-4422}} % 21505
% \author{S.~Bahinipati\,\orcidlink{0000-0002-3744-5332}} % 2332
% \author{A.~M.~Bakich\,\orcidlink{0000-0001-8315-4854}} % 2115
  \author{P.~Bambade\,\orcidlink{0000-0001-7378-4852}} % 3003
  \author{Sw.~Banerjee\,\orcidlink{0000-0001-8852-2409}} % 8603
  \author{S.~Bansal\,\orcidlink{0000-0003-1992-0336}} % 5163
  \author{M.~Barrett\,\orcidlink{0000-0002-2095-603X}} % 2180
  \author{M.~Bartl\,\orcidlink{0009-0002-7835-0855}} % 26483
% \author{G.~Batignani\,\orcidlink{0000-0003-3917-3104}} % 6643
  \author{J.~Baudot\,\orcidlink{0000-0001-5585-0991}} % 2562
% \author{M.~Bauer\,\orcidlink{0000-0002-0953-7387}} % 9863
  \author{A.~Baur\,\orcidlink{0000-0003-1360-3292}} % 5683
  \author{A.~Beaubien\,\orcidlink{0000-0001-9438-089X}} % 6683
  \author{F.~Becherer\,\orcidlink{0000-0003-0562-4616}} % 21623
  \author{J.~Becker\,\orcidlink{0000-0002-5082-5487}} % 5403
% \author{P.~K.~Behera\,\orcidlink{0000-0002-1527-2266}} % 4204
  \author{J.~V.~Bennett\,\orcidlink{0000-0002-5440-2668}} % 2454
% \author{E.~Bernieri\,\orcidlink{0000-0002-4787-2047}} % 4483
  \author{F.~U.~Bernlochner\,\orcidlink{0000-0001-8153-2719}} % 2282
  \author{V.~Bertacchi\,\orcidlink{0000-0001-9971-1176}} % 2212
  \author{M.~Bertemes\,\orcidlink{0000-0001-5038-360X}} % 2595
  \author{E.~Bertholet\,\orcidlink{0000-0002-3792-2450}} % 13163
  \author{M.~Bessner\,\orcidlink{0000-0003-1776-0439}} % 3783
% \author{D.~Z.~Besson\,\orcidlink{-}} % 3585
  \author{S.~Bettarini\,\orcidlink{0000-0001-7742-2998}} % 2350
  \author{V.~Bhardwaj\,\orcidlink{0000-0001-8857-8621}} % 2228
  \author{B.~Bhuyan\,\orcidlink{0000-0001-6254-3594}} % 2097
  \author{F.~Bianchi\,\orcidlink{0000-0002-1524-6236}} % 2564
% \author{L.~Bierwirth\,\orcidlink{0009-0003-0192-9073}} % 11723
% \author{T.~Bilka\,\orcidlink{0000-0003-1449-6986}} % 2484
% \author{S.~Bilokin\,\orcidlink{0000-0003-0017-6260}} % 3623
  \author{D.~Biswas\,\orcidlink{0000-0002-7543-3471}} % 8703
% \author{T.~Bloomfield\,\orcidlink{0000-0001-9288-5069}} % 2418
  \author{A.~Bobrov\,\orcidlink{0000-0001-5735-8386}} % 2294
  \author{D.~Bodrov\,\orcidlink{0000-0001-5279-4787}} % 9643
% \author{A.~Bolz\,\orcidlink{0000-0002-4033-9223}} % 15403
  \author{A.~Bondar\,\orcidlink{0000-0002-5089-5338}} % 4643
  \author{G.~Bonvicini\,\orcidlink{0000-0003-4861-7918}} % 2095
  \author{J.~Borah\,\orcidlink{0000-0003-2990-1913}} % 7083
  \author{A.~Boschetti\,\orcidlink{0000-0001-6030-3087}} % 17683
  \author{A.~Bozek\,\orcidlink{0000-0002-5915-1319}} % 2303
  \author{M.~Bra\v{c}ko\,\orcidlink{0000-0002-2495-0524}} % 2425
  \author{P.~Branchini\,\orcidlink{0000-0002-2270-9673}} % 2577
% \author{N.~Brenny\,\orcidlink{0009-0006-2917-9173}} % 19943
  \author{R.~A.~Briere\,\orcidlink{0000-0001-5229-1039}} % 2584
  \author{T.~E.~Browder\,\orcidlink{0000-0001-7357-9007}} % 2560
% \author{Y.~Buch\,\orcidlink{0000-0002-8050-4000}} % 17323
  \author{A.~Budano\,\orcidlink{0000-0002-0856-1131}} % 2171
  \author{S.~Bussino\,\orcidlink{0000-0002-3829-9592}} % 5384
% \author{A.~Calcaterra\,\orcidlink{0000-0003-2670-4826}} % 19163
% \author{A.~Caldwell\,\orcidlink{0000-0003-0244-5129}} % 2608
  \author{Q.~Campagna\,\orcidlink{0000-0002-3109-2046}} % 21563
  \author{M.~Campajola\,\orcidlink{0000-0003-2518-7134}} % 5223
  \author{L.~Cao\,\orcidlink{0000-0001-8332-5668}} % 2099
  \author{G.~Casarosa\,\orcidlink{0000-0003-4137-938X}} % 2491
  \author{C.~Cecchi\,\orcidlink{0000-0002-2192-8233}} % 2433
% \author{J.~Cerasoli\,\orcidlink{0000-0001-9777-881X}} % 20746
  \author{M.-C.~Chang\,\orcidlink{0000-0002-8650-6058}} % 2827
% \author{P.~Chang\,\orcidlink{0000-0003-4064-388X}} % 2542
% \author{R.~Cheaib\,\orcidlink{0000-0001-5729-8926}} % 2208
  \author{P.~Cheema\,\orcidlink{0000-0001-8472-5727}} % 15264
% \author{V.~Chekelian\,\orcidlink{0000-0001-8860-8288}} % 2167
% \author{C.~Chen\,\orcidlink{0000-0003-1589-9955}} % 12803
  \author{L.~Chen\,\orcidlink{0009-0003-6318-2008}} % 17363
% \author{Y.-T.~Chen\,\orcidlink{0000-0003-2639-2850}} % 2884
  \author{B.~G.~Cheon\,\orcidlink{0000-0002-8803-4429}} % 2173
% \author{C.~Cheshta\,\orcidlink{0009-0004-1205-5700}} % 25483
  \author{K.~Chilikin\,\orcidlink{0000-0001-7620-2053}} % 2308
  \author{J.~Chin\,\orcidlink{0009-0005-9210-8872}} % 20283
  \author{K.~Chirapatpimol\,\orcidlink{0000-0003-2099-7760}} % 10803
  \author{H.-E.~Cho\,\orcidlink{0000-0002-7008-3759}} % 2182
  \author{K.~Cho\,\orcidlink{0000-0003-1705-7399}} % 2516
  \author{S.-J.~Cho\,\orcidlink{0000-0002-1673-5664}} % 2723
  \author{S.-K.~Choi\,\orcidlink{0000-0003-2747-8277}} % 2364
  \author{S.~Choudhury\,\orcidlink{0000-0001-9841-0216}} % 2206
% \author{K.~Chu\,\orcidlink{0000-0002-1997-4249}} % 5203
% \author{D.~Cinabro\,\orcidlink{0000-0001-7347-6585}} % 2092
% \author{J.~Cochran\,\orcidlink{0000-0002-1492-914X}} % 12604
  \author{I.~Consigny\,\orcidlink{0009-0009-8755-6290}} % 23903
  \author{L.~Corona\,\orcidlink{0000-0002-2577-9909}} % 3944
% \author{L.~M.~Cremaldi\,\orcidlink{0000-0001-5550-7827}} % 2276
  \author{J.~X.~Cui\,\orcidlink{0000-0002-2398-3754}} % 8863
% \author{T.~Czank\,\orcidlink{0000-0001-6621-3373}} % 2254
  \author{S.~Das\,\orcidlink{0000-0001-6857-966X}} % 9163
% \author{F.~Dattola\,\orcidlink{0000-0003-3316-8574}} % 3745
  \author{E.~De~La~Cruz-Burelo\,\orcidlink{0000-0002-7469-6974}} % 2359
  \author{S.~A.~De~La~Motte\,\orcidlink{0000-0003-3905-6805}} % 2128
% \author{G.~de~Marino\,\orcidlink{0000-0002-6509-7793}} % 8364
% \author{G.~De~Nardo\,\orcidlink{0000-0002-2047-9675}} % 2459
% \author{M.~De~Nuccio\,\orcidlink{0000-0002-0972-9047}} % 2610
  \author{G.~De~Pietro\,\orcidlink{0000-0001-8442-107X}} % 2528
  \author{R.~de~Sangro\,\orcidlink{0000-0002-3808-5455}} % 2524
% \author{B.~Deschamps\,\orcidlink{0000-0003-2497-5008}} % 2671
  \author{M.~Destefanis\,\orcidlink{0000-0003-1997-6751}} % 2594
% \author{S.~Dey\,\orcidlink{0000-0003-2997-3829}} % 5023
% \author{A.~De~Yta-Hernandez\,\orcidlink{0000-0002-2162-7334}} % 2104
% \author{R.~Dhamija\,\orcidlink{0000-0001-7052-3163}} % 9465
  \author{A.~Di~Canto\,\orcidlink{0000-0003-1233-3876}} % 10963
% \author{F.~Di~Capua\,\orcidlink{0000-0001-9076-5936}} % 2065
% \author{J.~Dingfelder\,\orcidlink{0000-0001-5767-2121}} % 2151
  \author{Z.~Dole\v{z}al\,\orcidlink{0000-0002-5662-3675}} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez\,\orcidlink{0000-0001-6831-3159}} % 2191
  \author{T.~V.~Dong\,\orcidlink{0000-0003-3043-1939}} % 2215
  \author{X.~Dong\,\orcidlink{0000-0001-8574-9624}} % 17343
  \author{M.~Dorigo\,\orcidlink{0000-0002-0681-6946}} % 12543
% \author{D.~Dorner\,\orcidlink{0000-0003-3628-9267}} % 13564
% \author{K.~Dort\,\orcidlink{0000-0003-0849-8774}} % 5583
% \author{D.~Dossett\,\orcidlink{0000-0002-5670-5582}} % 2574
% \author{S.~Dreyer\,\orcidlink{0000-0002-6295-100X}} % 12823
% \author{S.~Dubey\,\orcidlink{0000-0002-1345-0970}} % 11063
% \author{S.~Duell\,\orcidlink{0000-0001-9918-9808}} % 2344
  \author{K.~Dugic\,\orcidlink{0009-0006-6056-546X}} % 11103
  \author{G.~Dujany\,\orcidlink{0000-0002-1345-8163}} % 9703
  \author{P.~Ecker\,\orcidlink{0000-0002-6817-6868}} % 5563
% \author{M.~Eliachevitch\,\orcidlink{0000-0003-2033-537X}} % 2725
  \author{D.~Epifanov\,\orcidlink{0000-0001-8656-2693}} % 2551
  \author{J.~Eppelt\,\orcidlink{0000-0001-8368-3721}} % 19723
% \author{Y.~Fan\,\orcidlink{0000-0001-9616-9705}} % 21303
  \author{R.~Farkas\,\orcidlink{0000-0002-7647-1429}} % 12843
  \author{P.~Feichtinger\,\orcidlink{0000-0003-3966-7497}} % 9843
  \author{T.~Ferber\,\orcidlink{0000-0002-6849-0427}} % 2482
% \author{D.~Ferlewicz\,\orcidlink{0000-0002-4374-1234}} % 2073
  \author{T.~Fillinger\,\orcidlink{0000-0001-9795-7412}} % 9803
  \author{C.~Finck\,\orcidlink{0000-0002-5068-5453}} % 15803
  \author{G.~Finocchiaro\,\orcidlink{0000-0002-3936-2151}} % 2400
% \author{P.~Fischer\,\orcidlink{0000-0002-9808-3574}} % 2141
% \author{K.~Flood\,\orcidlink{0000-0002-3463-6571}} % 12103
% \author{A.~Fodor\,\orcidlink{0000-0002-2821-759X}} % 2312
  \author{F.~Forti\,\orcidlink{0000-0001-6535-7965}} % 2432
  \author{A.~Frey\,\orcidlink{0000-0001-7470-3874}} % 2150
% \author{M.~Friedl\,\orcidlink{0000-0002-7420-2559}} % 2442
  \author{B.~G.~Fulsom\,\orcidlink{0000-0002-5862-9739}} % 2563
  \author{A.~Gabrielli\,\orcidlink{0000-0001-7695-0537}} % 13523
% \author{N.~Gabyshev\,\orcidlink{0000-0002-8593-6857}} % 2510
  \author{A.~Gale\,\orcidlink{0009-0005-2634-7189}} % 20263
  \author{E.~Ganiev\,\orcidlink{0000-0001-8346-8597}} % 4623
  \author{M.~Garcia-Hernandez\,\orcidlink{0000-0003-2393-3367}} % 4823
  \author{R.~Garg\,\orcidlink{0000-0002-7406-4707}} % 2213
% \author{A.~Garmash\,\orcidlink{0000-0003-2599-1405}} % 2161
% \author{L.~G\"artner\,\orcidlink{0000-0002-3643-4543}} % 21783
  \author{G.~Gaudino\,\orcidlink{0000-0001-5983-1552}} % 16563
  \author{V.~Gaur\,\orcidlink{0000-0002-8880-6134}} % 2413
  \author{V.~Gautam\,\orcidlink{0009-0001-9817-8637}} % 22223
  \author{A.~Gaz\,\orcidlink{0000-0001-6754-3315}} % 2181
  \author{A.~Gellrich\,\orcidlink{0000-0003-0974-6231}} % 2480
% \author{G.~Ghevondyan\,\orcidlink{0000-0003-0096-3555}} % 9445
  \author{D.~Ghosh\,\orcidlink{0000-0002-3458-9824}} % 11923
  \author{H.~Ghumaryan\,\orcidlink{0000-0001-6775-8893}} % 19543
  \author{G.~Giakoustidis\,\orcidlink{0000-0001-5982-1784}} % 13723
  \author{R.~Giordano\,\orcidlink{0000-0002-5496-7247}} % 2103
  \author{A.~Giri\,\orcidlink{0000-0002-8895-0128}} % 2106
  \author{P.~Gironella~Gironell\,\orcidlink{0000-0001-5603-4750}} % 25443
% \author{A.~Glazov\,\orcidlink{0000-0002-8553-7338}} % 2473
  \author{B.~Gobbo\,\orcidlink{0000-0002-3147-4562}} % 2109
  \author{R.~Godang\,\orcidlink{0000-0002-8317-0579}} % 2449
  \author{O.~Gogota\,\orcidlink{0000-0003-4108-7256}} % 2334
  \author{P.~Goldenzweig\,\orcidlink{0000-0001-8785-847X}} % 2345
% \author{B.~Golob\,\orcidlink{0000-0001-9632-5616}} % 3703
% \author{G.~Gong\,\orcidlink{0000-0001-7192-1833}} % 2727
% \author{P.~Grace\,\orcidlink{0000-0001-9005-7403}} % 9563
  \author{W.~Gradl\,\orcidlink{0000-0002-9974-8320}} % 2570
% \author{M.~Graf-Schreiber\,\orcidlink{0000-0003-4613-1041}} % 2730
% \author{T.~Grammatico\,\orcidlink{0000-0002-2818-9744}} % 20623
% \author{S.~Granderath\,\orcidlink{0000-0002-9945-463X}} % 8383
  \author{E.~Graziani\,\orcidlink{0000-0001-8602-5652}} % 2342
  \author{D.~Greenwald\,\orcidlink{0000-0001-6964-8399}} % 2686
% \author{T.~Gu\,\orcidlink{0000-0002-1470-6536}} % 14283
  \author{Y.~Guan\,\orcidlink{0000-0002-5541-2278}} % 2514
  \author{K.~Gudkova\,\orcidlink{0000-0002-5858-3187}} % 10504
  \author{I.~Haide\,\orcidlink{0000-0003-0962-6344}} % 14824
% \author{H.~Haigh\,\orcidlink{0000-0003-1567-0907}} % 16744
% \author{S.~Halder\,\orcidlink{0000-0002-6280-494X}} % 4743
% \author{Y.~Han\,\orcidlink{0000-0001-6775-5932}} % 19663
% \author{K.~Hara\,\orcidlink{0000-0002-5361-1871}} % 2462
% \author{T.~Hara\,\orcidlink{0000-0002-4321-0417}} % 2523
% \author{C.~Harris\,\orcidlink{0000-0003-0448-4244}} % 21383
% \author{K.~Hayasaka\,\orcidlink{0000-0002-6347-433X}} % 2330
  \author{H.~Hayashii\,\orcidlink{0000-0002-5138-5903}} % 2455
  \author{S.~Hazra\,\orcidlink{0000-0001-6954-9593}} % 7663
  \author{C.~Hearty\,\orcidlink{0000-0001-6568-0252}} % 2450
  \author{M.~T.~Hedges\,\orcidlink{0000-0001-6504-1872}} % 2265
  \author{A.~Heidelbach\,\orcidlink{0000-0002-6663-5469}} % 16923
  \author{G.~Heine\,\orcidlink{0009-0009-1827-2008}} % 23863
  \author{I.~Heredia~de~la~Cruz\,\orcidlink{0000-0002-8133-6467}} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva\,\orcidlink{0000-0002-6322-5587}} % 2466
  \author{T.~Higuchi\,\orcidlink{0000-0002-7761-3505}} % 2485
% \author{H.~Hirata\,\orcidlink{0000-0001-9005-4616}} % 2070
  \author{M.~Hoek\,\orcidlink{0000-0002-1893-8764}} % 2101
  \author{M.~Hohmann\,\orcidlink{0000-0001-5147-4781}} % 2077
  \author{R.~Hoppe\,\orcidlink{0009-0005-8881-8935}} % 23383
  \author{P.~Horak\,\orcidlink{0000-0001-9979-6501}} % 13583
% \author{T.~Hotta\,\orcidlink{0000-0002-1079-5826}} % 2084
  \author{C.-L.~Hsu\,\orcidlink{0000-0002-1641-430X}} % 2299
% \author{A.~Huang\,\orcidlink{0000-0003-1748-7348}} % 14223
% \author{K.~Huang\,\orcidlink{0000-0001-9342-7406}} % 2389
  \author{T.~Humair\,\orcidlink{0000-0002-2922-9779}} % 10643
  \author{T.~Iijima\,\orcidlink{0000-0002-4271-711X}} % 2446
  \author{K.~Inami\,\orcidlink{0000-0003-2765-7072}} % 2323
  \author{G.~Inguglia\,\orcidlink{0000-0003-0331-8279}} % 2500
  \author{N.~Ipsita\,\orcidlink{0000-0002-2927-3366}} % 12223
% \author{C.~Irmler\,\orcidlink{0009-0008-8290-8472}} % 2186
  \author{A.~Ishikawa\,\orcidlink{0000-0002-3561-5633}} % 2281
  \author{R.~Itoh\,\orcidlink{0000-0003-1590-0266}} % 2487
  \author{M.~Iwasaki\,\orcidlink{0000-0002-9402-7559}} % 2360
% \author{Y.~Iwasaki\,\orcidlink{0000-0001-7261-2557}} % 2229
% \author{S.~Iwata\,\orcidlink{0009-0005-5017-8098}} % 4323
% \author{P.~Jackson\,\orcidlink{0000-0002-0847-402X}} % 2255
  \author{D.~Jacobi\,\orcidlink{0000-0003-2399-9796}} % 15123
  \author{W.~W.~Jacobs\,\orcidlink{0000-0002-9996-6336}} % 2322
  \author{D.~E.~Jaffe\,\orcidlink{0000-0003-3122-4384}} % 3663
  \author{E.-J.~Jang\,\orcidlink{0000-0002-1935-9887}} % 6744
  \author{Q.~P.~Ji\,\orcidlink{0000-0003-2963-2565}} % 16243
% \author{X.~B.~Ji\,\orcidlink{0000-0002-6337-5040}} % 2558
  \author{S.~Jia\,\orcidlink{0000-0001-8176-8545}} % 2457
  \author{Y.~Jin\,\orcidlink{0000-0002-7323-0830}} % 2105
  \author{A.~Johnson\,\orcidlink{0000-0002-8366-1749}} % 16143
  \author{K.~K.~Joo\,\orcidlink{0000-0002-5515-0087}} % 4224
% \author{H.~Junkerkalefeld\,\orcidlink{0000-0003-3987-9895}} % 12963
% \author{I.~Kadenko\,\orcidlink{0000-0001-8766-4229}} % 3843
% \author{H.~Kakuno\,\orcidlink{0000-0002-9957-6055}} % 2391
% \author{M.~Kaleta\,\orcidlink{0000-0002-2863-5476}} % 5603
% \author{D.~Kalita\,\orcidlink{0000-0003-3054-1222}} % 2220
% \author{A.~B.~Kaliyar\,\orcidlink{0000-0002-2211-619X}} % 7344
  \author{J.~Kandra\,\orcidlink{0000-0001-5635-1000}} % 2541
  \author{K.~H.~Kang\,\orcidlink{0000-0002-6816-0751}} % 2283
% \author{S.~Kang\,\orcidlink{0000-0002-5320-7043}} % 12683
  \author{G.~Karyan\,\orcidlink{0000-0001-5365-3716}} % 2550
% \author{H.~Kawai\,\orcidlink{-}} % 4344
  \author{T.~Kawasaki\,\orcidlink{0000-0002-4089-5238}} % 4363
  \author{F.~Keil\,\orcidlink{0000-0002-7278-2860}} % 19523
  \author{C.~Ketter\,\orcidlink{0000-0002-5161-9722}} % 2236
% \author{M.~Khan\,\orcidlink{0000-0002-2168-0872}} % 15644
  \author{C.~Kiesling\,\orcidlink{0000-0002-2209-535X}} % 2168
% \author{C.~Kim\,\orcidlink{0009-0000-9835-9625}} % 20503
  \author{C.-H.~Kim\,\orcidlink{0000-0002-5743-7698}} % 2358
  \author{D.~Y.~Kim\,\orcidlink{0000-0001-8125-9070}} % 2315
  \author{J.-Y.~Kim\,\orcidlink{0000-0001-7593-843X}} % 20223
  \author{K.-H.~Kim\,\orcidlink{0000-0002-4659-1112}} % 2118
% \author{S.~K.~Kim\,\orcidlink{-}} % 3823
% \author{Y.~J.~Kim\,\orcidlink{0000-0001-9511-9634}} % 2403
  \author{Y.-K.~Kim\,\orcidlink{0000-0002-9695-8103}} % 2379
  \author{H.~Kindo\,\orcidlink{0000-0002-6756-3591}} % 2195
  \author{K.~Kinoshita\,\orcidlink{0000-0001-7175-4182}} % 2318
  \author{P.~Kody\v{s}\,\orcidlink{0000-0002-8644-2349}} % 2407
  \author{T.~Koga\,\orcidlink{0000-0002-1644-2001}} % 6963
  \author{S.~Kohani\,\orcidlink{0000-0003-3869-6552}} % 9143
  \author{K.~Kojima\,\orcidlink{0000-0002-3638-0266}} % 6363
% \author{T.~Konno\,\orcidlink{0000-0003-2487-8080}} % 2490
% \author{H.~Korandla\,\orcidlink{0000-0003-0516-7793}} % 18783
  \author{A.~Korobov\,\orcidlink{0000-0001-5959-8172}} % 4185
  \author{S.~Korpar\,\orcidlink{0000-0003-0971-0968}} % 2475
% \author{E.~Kou\,\orcidlink{0000-0002-8650-6699}} % 3765
  \author{E.~Kovalenko\,\orcidlink{0000-0001-8084-1931}} % 3884
  \author{R.~Kowalewski\,\orcidlink{0000-0002-7314-0990}} % 2293
% \author{T.~M.~G.~Kraetzschmar\,\orcidlink{0000-0001-8395-2928}} % 7543
  \author{P.~Kri\v{z}an\,\orcidlink{0000-0002-4967-7675}} % 2474
% \author{R.~Kroeger\,\orcidlink{-}} % 2242
  \author{P.~Krokovny\,\orcidlink{0000-0002-1236-4667}} % 2575
% \author{W.~Kuehn\,\orcidlink{0000-0001-6018-9878}} % 2534
% \author{T.~Kuhr\,\orcidlink{0000-0001-6251-8049}} % 2486
  \author{Y.~Kulii\,\orcidlink{0000-0001-6217-5162}} % 9823
% \author{D.~Kumar\,\orcidlink{0000-0001-6585-7767}} % 7223
% \author{J.~Kumar\,\orcidlink{0000-0002-8465-433X}} % 6464
% \author{M.~Kumar\,\orcidlink{0000-0002-6627-9708}} % 2744
  \author{R.~Kumar\,\orcidlink{0000-0002-6277-2626}} % 2189
  \author{K.~Kumara\,\orcidlink{0000-0003-1572-5365}} % 2257
% \author{T.~Kumita\,\orcidlink{0000-0001-7572-4538}} % 4083
  \author{T.~Kunigo\,\orcidlink{0000-0001-9613-2849}} % 10104
% \author{A.~Kusudo\,\orcidlink{0000-0002-2662-9734}} % 14623
  \author{A.~Kuzmin\,\orcidlink{0000-0002-7011-5044}} % 2520
% \author{P.~Kvasni\v{c}ka\,\orcidlink{0000-0001-6281-0648}} % 2184
  \author{Y.-J.~Kwon\,\orcidlink{0000-0001-9448-5691}} % 2231
% \author{S.~Lacaprara\,\orcidlink{0000-0002-0551-7696}} % 2447
% \author{Y.-T.~Lai\,\orcidlink{0000-0001-9553-3421}} % 2066
  \author{K.~Lalwani\,\orcidlink{0000-0002-7294-396X}} % 2142
  \author{T.~Lam\,\orcidlink{0000-0001-9128-6806}} % 2729
  \author{L.~Lanceri\,\orcidlink{0000-0001-8220-3095}} % 2540
  \author{J.~S.~Lange\,\orcidlink{0000-0003-0234-0474}} % 2277
  \author{T.~S.~Lau\,\orcidlink{0000-0001-7110-7823}} % 19803
  \author{M.~Laurenza\,\orcidlink{0000-0002-7400-6013}} % 10223
% \author{K.~Lautenbach\,\orcidlink{0000-0003-3762-694X}} % 2102
% \author{P.~J.~Laycock\,\orcidlink{0000-0002-8572-5339}} % 7683
  \author{R.~Leboucher\,\orcidlink{0000-0003-3097-6613}} % 14083
  \author{F.~R.~Le~Diberder\,\orcidlink{0000-0002-9073-5689}} % 3267
  \author{M.~J.~Lee\,\orcidlink{0000-0003-4528-4601}} % 21803
% \author{P.~Leitl\,\orcidlink{0000-0002-1336-9558}} % 2414
  \author{C.~Lemettais\,\orcidlink{0009-0008-5394-5100}} % 22704
  \author{P.~Leo\,\orcidlink{0000-0003-3833-2900}} % 19823
% \author{D.~Levit\,\orcidlink{0000-0001-5789-6205}} % 2507
  \author{P.~M.~Lewis\,\orcidlink{0000-0002-5991-622X}} % 2582
  \author{C.~Li\,\orcidlink{0000-0002-3240-4523}} % 2325
  \author{H.-J.~Li\,\orcidlink{0000-0001-9275-4739}} % 4943
  \author{L.~K.~Li\,\orcidlink{0000-0002-7366-1307}} % 3263
% \author{Q.~M.~Li\,\orcidlink{0009-0004-9425-2678}} % 22943
  \author{S.~X.~Li\,\orcidlink{0000-0003-4669-1495}} % 2377
  \author{W.~Z.~Li\,\orcidlink{0009-0002-8040-2546}} % 19703
  \author{Y.~Li\,\orcidlink{0000-0002-4413-6247}} % 8083
  \author{Y.~B.~Li\,\orcidlink{0000-0002-9909-2851}} % 2573
  \author{Y.~P.~Liao\,\orcidlink{0009-0000-1981-0044}} % 24303
  \author{J.~Libby\,\orcidlink{0000-0002-1219-3247}} % 2262
  \author{J.~Lin\,\orcidlink{0000-0002-3653-2899}} % 2401
  \author{S.~Lin\,\orcidlink{0000-0001-5922-9561}} % 17223
% \author{Z.~Liptak\,\orcidlink{0000-0002-6491-8131}} % 3565
% \author{V.~Lisovskyi\,\orcidlink{0000-0003-4451-214X}} % 26584
% \author{A.~Little\,\orcidlink{0009-0008-4974-3661}} % 23803
  \author{M.~H.~Liu\,\orcidlink{0000-0002-9376-1487}} % 15244
  \author{Q.~Y.~Liu\,\orcidlink{0000-0002-7684-0415}} % 7045
  \author{Y.~Liu\,\orcidlink{0000-0002-8374-3947}} % 16223
  \author{Z.~Liu\,\orcidlink{0000-0002-0290-3022}} % 11303
% \author{Z.~A.~Liu\,\orcidlink{0000-0002-2896-1386}} % 3283
  \author{D.~Liventsev\,\orcidlink{0000-0003-3416-0056}} % 2578
  \author{S.~Longo\,\orcidlink{0000-0002-8124-8969}} % 2396
% \author{G.~Lopez-Castro\,\orcidlink{-}} % 4245
  \author{A.~Lozar\,\orcidlink{0000-0002-0569-6882}} % 12423
  \author{T.~Lueck\,\orcidlink{0000-0003-3915-2506}} % 2406
% \author{T.~Luo\,\orcidlink{0000-0001-5139-5784}} % 3268
  \author{C.~Lyu\,\orcidlink{0000-0002-2275-0473}} % 12484
  \author{Y.~Ma\,\orcidlink{0000-0001-8412-8308}} % 16883
% \author{A.~Maeda\,\orcidlink{0009-0009-8839-7148}} % 14664
  \author{M.~Maggiora\,\orcidlink{0000-0003-4143-9127}} % 5343
  \author{S.~P.~Maharana\,\orcidlink{0000-0002-1746-4683}} % 19083
% \author{T.~Mahood\,\orcidlink{0009-0004-3017-6661}} % 26003
  \author{R.~Maiti\,\orcidlink{0000-0001-5534-7149}} % 12043
% \author{S.~Maity\,\orcidlink{0000-0003-3076-9243}} % 2985
  \author{G.~Mancinelli\,\orcidlink{0000-0003-1144-3678}} % 20743
  \author{R.~Manfredi\,\orcidlink{0000-0002-8552-6276}} % 10303
  \author{E.~Manoni\,\orcidlink{0000-0002-9826-7947}} % 2305
% \author{A.~C.~Manthei\,\orcidlink{0000-0002-6900-5729}} % 15023
  \author{M.~Mantovano\,\orcidlink{0000-0002-5979-5050}} % 19783
  \author{D.~Marcantonio\,\orcidlink{0000-0002-1315-8646}} % 11163
  \author{S.~Marcello\,\orcidlink{0000-0003-4144-863X}} % 4223
  \author{C.~Marinas\,\orcidlink{0000-0003-1903-3251}} % 2133
  \author{C.~Martellini\,\orcidlink{0000-0002-7189-8343}} % 16983
  \author{A.~Martens\,\orcidlink{0000-0003-1544-4053}} % 13823
% \author{A.~Martini\,\orcidlink{0000-0003-1161-4983}} % 2336
  \author{T.~Martinov\,\orcidlink{0000-0001-7846-1913}} % 19463
  \author{L.~Massaccesi\,\orcidlink{0000-0003-1762-4699}} % 16323
  \author{M.~Masuda\,\orcidlink{0000-0002-7109-5583}} % 2238
% \author{T.~Matsuda\,\orcidlink{0000-0003-4673-570X}} % 5543
% \author{K.~Matsuoka\,\orcidlink{0000-0003-1706-9365}} % 2316
  \author{D.~Matvienko\,\orcidlink{0000-0002-2698-5448}} % 2351
  \author{S.~K.~Maurya\,\orcidlink{0000-0002-7764-5777}} % 9763
  \author{M.~Maushart\,\orcidlink{0009-0004-1020-7299}} % 21203
% \author{F.~Mawas\,\orcidlink{0000-0002-7176-4732}} % 20943
  \author{J.~A.~McKenna\,\orcidlink{0000-0001-9871-9002}} % 2392
  \author{Z.~Mediankin~Gruberov\'{a}\,\orcidlink{0000-0002-5691-1044}} % 8824
% \author{F.~Meggendorfer\,\orcidlink{0000-0002-1466-7207}} % 7103
  \author{R.~Mehta\,\orcidlink{0000-0001-8670-3409}} % 15203
  \author{F.~Meier\,\orcidlink{0000-0002-6088-0412}} % 3103
  \author{D.~Meleshko\,\orcidlink{0000-0002-0872-4623}} % 11523
  \author{M.~Merola\,\orcidlink{0000-0002-7082-8108}} % 2456
% \author{F.~Metzner\,\orcidlink{0000-0002-0128-264X}} % 2296
% \author{M.~Milesi\,\orcidlink{0000-0002-8805-1886}} % 5443
  \author{C.~Miller\,\orcidlink{0000-0003-2631-1790}} % 2273
  \author{M.~Mirra\,\orcidlink{0000-0002-1190-2961}} % 14744
  \author{S.~Mitra\,\orcidlink{0000-0002-1118-6344}} % 19944
  \author{K.~Miyabayashi\,\orcidlink{0000-0003-4352-734X}} % 2327
% \author{H.~Miyake\,\orcidlink{0000-0002-7079-8236}} % 2452
% \author{R.~Mizuk\,\orcidlink{0000-0002-2209-6969}} % 2483
  \author{G.~B.~Mohanty\,\orcidlink{0000-0001-6850-7666}} % 2278
  \author{S.~Mondal\,\orcidlink{0000-0002-3054-8400}} % 19743
  \author{S.~Moneta\,\orcidlink{0000-0003-2184-7510}} % 13303
% \author{H.~Moon\,\orcidlink{0000-0001-5213-6477}} % 2304
  \author{A.~L.~Moreira~de~Carvalho\,\orcidlink{0000-0002-1986-5720}} % 26403
  \author{H.-G.~Moser\,\orcidlink{0000-0003-3579-9951}} % 2120
% \author{M.~Mrvar\,\orcidlink{0000-0001-6388-3005}} % 2527
% \author{Th.~Muller\,\orcidlink{0000-0003-4337-0098}} % 2165
  \author{R.~Mussa\,\orcidlink{0000-0002-0294-9071}} % 2372
  \author{I.~Nakamura\,\orcidlink{0000-0002-7640-5456}} % 3463
% \author{K.~R.~Nakamura\,\orcidlink{0000-0001-7012-7355}} % 2417
% \author{E.~Nakano\,\orcidlink{0000-0003-2282-5217}} % 2554
% \author{T.~Nakano\,\orcidlink{0000-0003-3157-5328}} % 2983
  \author{M.~Nakao\,\orcidlink{0000-0001-8424-7075}} % 2498
% \author{H.~Nakayama\,\orcidlink{0000-0002-2030-9967}} % 2232
% \author{H.~Nakazawa\,\orcidlink{0000-0003-1684-6628}} % 2335
  \author{Y.~Nakazawa\,\orcidlink{0000-0002-6271-5808}} % 17383
% \author{A.~Narimani~Charan\,\orcidlink{0000-0002-5975-550X}} % 10143
  \author{M.~Naruki\,\orcidlink{0000-0003-1773-2999}} % 4583
  \author{Z.~Natkaniec\,\orcidlink{0000-0003-0486-9291}} % 3923
  \author{A.~Natochii\,\orcidlink{0000-0002-1076-814X}} % 12063
% \author{L.~Nayak\,\orcidlink{0000-0002-7739-914X}} % 9464
  \author{M.~Nayak\,\orcidlink{0000-0002-2572-4692}} % 2371
% \author{G.~Nazaryan\,\orcidlink{0000-0002-9434-6197}} % 9523
  \author{M.~Neu\,\orcidlink{0000-0002-4564-8009}} % 23304
% \author{C.~Niebuhr\,\orcidlink{0000-0002-4375-9741}} % 2477
% \author{M.~Niiyama\,\orcidlink{0000-0003-1746-586X}} % 2063
% \author{J.~Ninkovic\,\orcidlink{0000-0003-1523-3635}} % 2386
  \author{S.~Nishida\,\orcidlink{0000-0001-6373-2346}} % 2571
% \author{K.~Nishimura\,\orcidlink{0000-0001-8818-8922}} % 3063
% \author{A.~Novosel\,\orcidlink{0000-0002-7308-8950}} % 15523
% \author{S.~Ogawa\,\orcidlink{0000-0002-7310-5079}} % 6263
  \author{R.~Okubo\,\orcidlink{0009-0009-0912-0678}} % 10743
% \author{S.~L.~Olsen\,\orcidlink{0000-0002-6388-9885}} % 4563
  \author{H.~Ono\,\orcidlink{0000-0003-4486-0064}} % 2160
  \author{Y.~Onuki\,\orcidlink{0000-0002-1646-6847}} % 2331
% \author{P.~Oskin\,\orcidlink{0000-0002-7524-0936}} % 9623
% \author{F.~Otani\,\orcidlink{0000-0001-6016-219X}} % 16244
  \author{E.~R.~Oxford\,\orcidlink{0000-0002-0813-4578}} % 6943
% \author{H.~Ozaki\,\orcidlink{0000-0001-6901-1881}} % 2984
% \author{P.~Pakhlov\,\orcidlink{0000-0001-7426-4824}} % 2221
  \author{G.~Pakhlova\,\orcidlink{0000-0001-7518-3022}} % 2188
% \author{A.~Panta\,\orcidlink{0000-0001-6385-7712}} % 7943
% \author{E.~Paoloni\,\orcidlink{0000-0001-5969-8712}} % 2488
  \author{S.~Pardi\,\orcidlink{0000-0001-7994-0537}} % 2532
  \author{K.~Parham\,\orcidlink{0000-0001-9556-2433}} % 10684
  \author{H.~Park\,\orcidlink{0000-0001-6087-2052}} % 2284
  \author{J.~Park\,\orcidlink{0000-0001-6520-0028}} % 18203
% \author{K.~Park\,\orcidlink{0000-0003-0567-3493}} % 12243
  \author{S.-H.~Park\,\orcidlink{0000-0001-6019-6218}} % 2509
  \author{B.~Paschen\,\orcidlink{0000-0003-1546-4548}} % 2159
  \author{A.~Passeri\,\orcidlink{0000-0003-4864-3411}} % 2116
  \author{S.~Patra\,\orcidlink{0000-0002-4114-1091}} % 3123
  \author{S.~Paul\,\orcidlink{0000-0002-8813-0437}} % 2131
  \author{T.~K.~Pedlar\,\orcidlink{0000-0001-9839-7373}} % 2421
  \author{I.~Peruzzi\,\orcidlink{0000-0001-6729-8436}} % 2253
% \author{R.~Peschke\,\orcidlink{0000-0002-2529-8515}} % 7123
  \author{R.~Pestotnik\,\orcidlink{0000-0003-1804-9470}} % 2476
% \author{F.~Pham\,\orcidlink{0000-0003-0608-2302}} % 2963
% \author{M.~Piccolo\,\orcidlink{0000-0001-9750-0551}} % 2147
  \author{L.~E.~Piilonen\,\orcidlink{0000-0001-6836-0748}} % 2346
  \author{P.~L.~M.~Podesta-Lerma\,\orcidlink{0000-0002-8152-9605}} % 2266
  \author{T.~Podobnik\,\orcidlink{0000-0002-6131-819X}} % 11223
% \author{S.~Pokharel\,\orcidlink{0000-0002-3367-738X}} % 12283
% \author{V.~Popov\,\orcidlink{0000-0003-0208-2583}} % 2096
  \author{A.~Prakash\,\orcidlink{0000-0002-6462-8142}} % 21663
  \author{C.~Praz\,\orcidlink{0000-0002-6154-885X}} % 2726
  \author{S.~Prell\,\orcidlink{0000-0002-0195-8005}} % 12743
  \author{E.~Prencipe\,\orcidlink{0000-0002-9465-2493}} % 2219
  \author{M.~T.~Prim\,\orcidlink{0000-0002-1407-7450}} % 2501
  \author{S.~Privalov\,\orcidlink{0009-0004-1681-3919}} % 12503
% \author{I.~Prudiiev\,\orcidlink{0000-0002-0819-284X}} % 19383
% \author{M.~V.~Purohit\,\orcidlink{0000-0002-8381-8689}} % 2196
  \author{H.~Purwar\,\orcidlink{0000-0002-3876-7069}} % 12363
% \author{N.~Rad\,\orcidlink{0000-0002-5204-0851}} % 11683
  \author{P.~Rados\,\orcidlink{0000-0003-0690-8100}} % 7383
  \author{G.~Raeuber\,\orcidlink{0000-0003-2948-5155}} % 18143
  \author{S.~Raiz\,\orcidlink{0000-0001-7010-8066}} % 13003
  \author{V.~Raj\,\orcidlink{0009-0003-2433-8065}} % 24983
% \author{N.~Rauls\,\orcidlink{0000-0002-6583-4888}} % 11603
  \author{K.~Ravindran\,\orcidlink{0000-0002-5584-2614}} % 22503
  \author{J.~U.~Rehman\,\orcidlink{0000-0002-2673-1982}} % 19623
  \author{M.~Reif\,\orcidlink{0000-0002-0706-0247}} % 8043
  \author{S.~Reiter\,\orcidlink{0000-0002-6542-9954}} % 2248
  \author{M.~Remnev\,\orcidlink{0000-0001-6975-1724}} % 2785
  \author{L.~Reuter\,\orcidlink{0000-0002-5930-6237}} % 16403
  \author{D.~Ricalde~Herrmann\,\orcidlink{0000-0001-9772-9989}} % 9263
  \author{I.~Ripp-Baudot\,\orcidlink{0000-0002-1897-8272}} % 2469
% \author{M.~Ritzert\,\orcidlink{0000-0003-2928-7044}} % 2526
  \author{G.~Rizzo\,\orcidlink{0000-0003-1788-2866}} % 2579
% \author{L.~B.~Rizzuto\,\orcidlink{0000-0001-6621-6646}} % 3746
  \author{S.~H.~Robertson\,\orcidlink{0000-0003-4096-8393}} % 2471
% \author{P.~Rocchetti\,\orcidlink{0000-0002-2839-3489}} % 13763
% \author{D.~Rodr\'{i}guez~P\'{e}rez\,\orcidlink{0000-0001-8505-649X}} % 2176
% \author{M.~Roehrken\,\orcidlink{0000-0003-0654-2866}} % 11883
  \author{J.~M.~Roney\,\orcidlink{0000-0001-7802-4617}} % 2244
% \author{C.~Rosenfeld\,\orcidlink{0000-0003-3857-1223}} % 2082
  \author{A.~Rostomyan\,\orcidlink{0000-0003-1839-8152}} % 2481
  \author{N.~Rout\,\orcidlink{0000-0002-4310-3638}} % 2965
% \author{M.~Rozanska\,\orcidlink{0000-0003-2651-5021}} % 2205
% \author{G.~Russo\,\orcidlink{0000-0001-5823-4393}} % 2388
% \author{D.~Sahoo\,\orcidlink{0000-0002-5600-9413}} % 2110
% \author{Y.~Sakai\,\orcidlink{0000-0001-9163-3409}} % 2175
% \author{L.~Salutari\,\orcidlink{0009-0001-2822-6939}} % 17423
% \author{G.~Sanchez\,\orcidlink{0000-0003-4824-9983}} % 2943
  \author{D.~A.~Sanders\,\orcidlink{0000-0002-4902-966X}} % 2458
  \author{S.~Sandilya\,\orcidlink{0000-0002-4199-4369}} % 2286
% \author{A.~Sangal\,\orcidlink{0000-0001-5853-349X}} % 2384
  \author{L.~Santelj\,\orcidlink{0000-0003-3904-2956}} % 2185
  \author{C.~Santos\,\orcidlink{0009-0005-2430-1670}} % 23743
% \author{Y.~Sato\,\orcidlink{0000-0003-3751-2803}} % 5243
  \author{V.~Savinov\,\orcidlink{0000-0002-9184-2830}} % 2292
  \author{B.~Scavino\,\orcidlink{0000-0003-1771-9161}} % 2518
  \author{C.~Schmitt\,\orcidlink{0000-0002-3787-687X}} % 15063
% \author{J.~Schmitz\,\orcidlink{0000-0001-8274-8124}} % 12863
% \author{S.~Schneider\,\orcidlink{0009-0002-5899-0353}} % 16803
  \author{M.~Schnepf\,\orcidlink{0000-0003-0623-0184}} % 15683
  \author{K.~Schoenning\,\orcidlink{0000-0002-3490-9584}} % 22023
% \author{J.~Schueler\,\orcidlink{0000-0002-2722-6953}} % 2824
  \author{C.~Schwanda\,\orcidlink{0000-0003-4844-5028}} % 2108
  \author{A.~J.~Schwartz\,\orcidlink{0000-0002-7310-1983}} % 2162
% \author{B.~Schwenker\,\orcidlink{0000-0002-7120-3732}} % 2405
% \author{M.~Schwickardi\,\orcidlink{0000-0003-2033-6700}} % 14743
  \author{Y.~Seino\,\orcidlink{0000-0002-8378-4255}} % 2517
  \author{A.~Selce\,\orcidlink{0000-0001-8228-9781}} % 9043
  \author{K.~Senyo\,\orcidlink{0000-0002-1615-9118}} % 2987
  \author{J.~Serrano\,\orcidlink{0000-0003-2489-7812}} % 12124
  \author{M.~E.~Sevior\,\orcidlink{0000-0002-4824-101X}} % 2328
  \author{C.~Sfienti\,\orcidlink{0000-0002-5921-8819}} % 2214
  \author{W.~Shan\,\orcidlink{0000-0003-2811-2218}} % 11943
% \author{C.~Sharma\,\orcidlink{0000-0002-1312-0429}} % 11584
  \author{G.~Sharma\,\orcidlink{0000-0002-5620-5334}} % 18423
% \author{V.~Shebalin\,\orcidlink{0000-0003-1012-0957}} % 2339
% \author{C.~P.~Shen\,\orcidlink{0000-0002-9012-4618}} % 2464
  \author{X.~D.~Shi\,\orcidlink{0000-0002-7006-6107}} % 18843
% \author{H.~Shibuya\,\orcidlink{0000-0002-0197-6270}} % 2234
  \author{T.~Shillington\,\orcidlink{0000-0003-3862-4380}} % 7983
  \author{T.~Shimasaki\,\orcidlink{0000-0003-3291-9532}} % 16263
% \author{M.~Shimomura\,\orcidlink{0000-0001-9598-779X}} % 2112
  \author{J.-G.~Shiu\,\orcidlink{0000-0002-8478-5639}} % 2412
  \author{D.~Shtol\,\orcidlink{0000-0002-0622-6065}} % 9223
  \author{B.~Shwartz\,\orcidlink{0000-0002-1456-1496}} % 2122
  \author{A.~Sibidanov\,\orcidlink{0000-0001-8805-4895}} % 2419
  \author{F.~Simon\,\orcidlink{0000-0002-5978-0289}} % 2164
% \author{J.~B.~Singh\,\orcidlink{0000-0001-9029-2462}} % 2903
  \author{J.~Skorupa\,\orcidlink{0000-0002-8566-621X}} % 12523
% \author{K.~Smith\,\orcidlink{0000-0003-0446-9474}} % 2243
  \author{R.~J.~Sobie\,\orcidlink{0000-0001-7430-7599}} % 2472
  \author{M.~Sobotzik\,\orcidlink{0000-0002-1773-5455}} % 8604
  \author{A.~Soffer\,\orcidlink{0000-0002-0749-2146}} % 2217
  \author{A.~Sokolov\,\orcidlink{0000-0002-9420-0091}} % 2521
% \author{Y.~Soloviev\,\orcidlink{0000-0003-1136-2827}} % 2479
  \author{E.~Solovieva\,\orcidlink{0000-0002-5735-4059}} % 2398
% \author{W.~Song\,\orcidlink{0000-0003-1376-2293}} % 22863
  \author{S.~Spataro\,\orcidlink{0000-0001-9601-405X}} % 2117
  \author{B.~Spruck\,\orcidlink{0000-0002-3060-2729}} % 2493
% \author{S.~Stani\v{c}\,\orcidlink{0000-0003-3344-8381}} % 3383
  \author{M.~Stari\v{c}\,\orcidlink{0000-0001-8751-5944}} % 2326
  \author{P.~Stavroulakis\,\orcidlink{0000-0001-9914-7261}} % 20643
  \author{S.~Stefkova\,\orcidlink{0000-0003-2628-530X}} % 8783
  \author{L.~Stoetzer\,\orcidlink{0009-0003-2245-1603}} % 19283
% \author{Z.~S.~Stottler\,\orcidlink{0000-0002-1898-5333}} % 2267
  \author{R.~Stroili\,\orcidlink{0000-0002-3453-142X}} % 2465
% \author{J.~Strube\,\orcidlink{0000-0001-7470-9301}} % 2451
% \author{J.~Su\,\orcidlink{0009-0001-1644-8198}} % 16623
% \author{Y.~Sue\,\orcidlink{0000-0003-2430-8707}} % 2085
% \author{R.~Sugiura\,\orcidlink{0000-0002-6044-5445}} % 4644
  \author{M.~Sumihama\,\orcidlink{0000-0002-8954-0585}} % 4243
% \author{K.~Sumisawa\,\orcidlink{0000-0001-7003-7210}} % 2583
% \author{W.~Sutcliffe\,\orcidlink{0000-0002-9795-3582}} % 3784
% \author{N.~Suwonjandee\,\orcidlink{0009-0000-2819-5020}} % 14063
  \author{H.~Svidras\,\orcidlink{0000-0003-4198-2517}} % 11783
% \author{M.~Takahashi\,\orcidlink{0000-0003-1171-5960}} % 2467
  \author{M.~Takizawa\,\orcidlink{0000-0001-8225-3973}} % 2437
% \author{U.~Tamponi\,\orcidlink{0000-0001-6651-0706}} % 2366
% \author{S.~Tanaka\,\orcidlink{0000-0002-6029-6216}} % 2530
  \author{S.~S.~Tang\,\orcidlink{0000-0001-6564-0445}} % 12003
  \author{K.~Tanida\,\orcidlink{0000-0002-8255-3746}} % 3803
% \author{H.~Tanigawa\,\orcidlink{0000-0003-3681-9985}} % 2237
% \author{N.~Taniguchi\,\orcidlink{0000-0002-1462-0564}} % 2285
  \author{F.~Tenchini\,\orcidlink{0000-0003-3469-9377}} % 2546
  \author{F.~Testa\,\orcidlink{0009-0004-5075-8247}} % 14844
% \author{A.~Thaller\,\orcidlink{0000-0003-4171-6219}} % 16044
  \author{O.~Tittel\,\orcidlink{0000-0001-9128-6240}} % 8663
  \author{R.~Tiwary\,\orcidlink{0000-0002-5887-1883}} % 10403
  \author{D.~Tonelli\,\orcidlink{0000-0002-1494-7882}} % 4564
  \author{E.~Torassa\,\orcidlink{0000-0003-2321-0599}} % 2556
% \author{N.~Toutounji\,\orcidlink{0000-0002-1937-6732}} % 2263
  \author{K.~Trabelsi\,\orcidlink{0000-0001-6567-3036}} % 2369
  \author{F.~F.~Trantou\,\orcidlink{0000-0003-0517-9129}} % 23643
  \author{I.~Tsaklidis\,\orcidlink{0000-0003-3584-4484}} % 13443
% \author{T.~Tsuboyama\,\orcidlink{0000-0002-4575-1997}} % 2361
% \author{N.~Tsuzuki\,\orcidlink{0000-0003-1141-1908}} % 2352
  \author{M.~Uchida\,\orcidlink{0000-0003-4904-6168}} % 2370
  \author{I.~Ueda\,\orcidlink{0000-0002-6833-4344}} % 2519
% \author{S.~Uehara\,\orcidlink{0000-0001-7377-5016}} % 2586
% \author{Y.~Uematsu\,\orcidlink{0000-0002-0296-4028}} % 5883
% \author{E.~Uenlue\,\orcidlink{0009-0000-3417-6790}} % 22283
  \author{T.~Uglov\,\orcidlink{0000-0002-4944-1830}} % 2252
  \author{K.~Unger\,\orcidlink{0000-0001-7378-6671}} % 9463
  \author{Y.~Unno\,\orcidlink{0000-0003-3355-765X}} % 2420
  \author{K.~Uno\,\orcidlink{0000-0002-2209-8198}} % 14963
  \author{S.~Uno\,\orcidlink{0000-0002-3401-0480}} % 2149
  \author{P.~Urquijo\,\orcidlink{0000-0002-0887-7953}} % 2302
  \author{Y.~Ushiroda\,\orcidlink{0000-0003-3174-403X}} % 2317
% \author{Y.~V.~Usov\,\orcidlink{0000-0003-3144-2920}} % 5003
  \author{S.~E.~Vahsen\,\orcidlink{0000-0003-1685-9824}} % 2251
  \author{R.~van~Tonder\,\orcidlink{0000-0002-7448-4816}} % 2706
  \author{K.~E.~Varvell\,\orcidlink{0000-0003-1017-1295}} % 2545
  \author{M.~Veronesi\,\orcidlink{0000-0002-1916-3884}} % 20723
% \author{A.~Vinokurova\,\orcidlink{0000-0003-4220-8056}} % 2289
  \author{V.~S.~Vismaya\,\orcidlink{0000-0002-1606-5349}} % 16063
  \author{L.~Vitale\,\orcidlink{0000-0003-3354-2300}} % 2415
% \author{V.~Vobbilisetti\,\orcidlink{0000-0002-4399-5082}} % 7364
  \author{R.~Volpe\,\orcidlink{0000-0003-1782-2978}} % 20183
% \author{A.~Vossen\,\orcidlink{0000-0003-0983-4936}} % 2249
% \author{B.~Wach\,\orcidlink{0000-0003-3533-7669}} % 8203
% \author{E.~Waheed\,\orcidlink{0000-0001-7774-0363}} % 2226
  \author{M.~Wakai\,\orcidlink{0000-0003-2818-3155}} % 3583
% \author{H.~M.~Wakeling\,\orcidlink{0000-0003-4606-7895}} % 3664
  \author{S.~Wallner\,\orcidlink{0000-0002-9105-1625}} % 20363
% \author{W.~Wan~Abdullah\,\orcidlink{0000-0001-5798-9145}} % 2280
% \author{B.~Wang\,\orcidlink{0000-0001-6136-6952}} % 2569
% \author{E.~Wang\,\orcidlink{0000-0001-6391-5118}} % 10983
% \author{L.~Wang\,\orcidlink{0000-0003-2464-6239}} % 22443
  \author{M.-Z.~Wang\,\orcidlink{0000-0002-0979-8341}} % 2074
  \author{X.~L.~Wang\,\orcidlink{0000-0001-5805-1255}} % 2076
% \author{Z.~Wang\,\orcidlink{0000-0002-3536-4950}} % 15743
  \author{A.~Warburton\,\orcidlink{0000-0002-2298-7315}} % 2347
% \author{M.~Watanabe\,\orcidlink{0000-0001-6917-6694}} % 2309
  \author{S.~Watanuki\,\orcidlink{0000-0002-5241-6628}} % 6843
% \author{M.~Welsch\,\orcidlink{0000-0002-3026-1872}} % 7023
% \author{O.~Werbycka\,\orcidlink{0000-0002-0614-8773}} % 6123
  \author{C.~Wessel\,\orcidlink{0000-0003-0959-4784}} % 2100
% \author{J.~Wiechczynski\,\orcidlink{0000-0002-3151-6072}} % 2604
  \author{E.~Won\,\orcidlink{0000-0002-4245-7442}} % 2410
% \author{L.~J.~Wu\,\orcidlink{0000-0002-3171-2436}} % 2704
% \author{Y.~Xie\,\orcidlink{0000-0002-0170-2798}} % 20383
% \author{X.~P.~Xu\,\orcidlink{0000-0001-5096-1182}} % 4923
% \author{Z.~Xu\,\orcidlink{0009-0005-1048-4744}} % 27103
  \author{B.~D.~Yabsley\,\orcidlink{0000-0002-2680-0474}} % 3645
  \author{S.~Yamada\,\orcidlink{0000-0002-8858-9336}} % 2492
  \author{W.~Yan\,\orcidlink{0000-0003-0713-0871}} % 2094
% \author{W.~C.~Yan\,\orcidlink{0000-0001-6721-9435}} % 2183
  \author{S.~B.~Yang\,\orcidlink{0000-0002-9543-7971}} % 2374
  \author{J.~Yelton\,\orcidlink{0000-0001-8840-3346}} % 2067
  \author{K.~Yi\,\orcidlink{0000-0002-2459-1824}} % 12583
  \author{J.~H.~Yin\,\orcidlink{0000-0002-1479-9349}} % 2365
% \author{Y.~M.~Yook\,\orcidlink{0000-0002-4912-048X}} % 2453
  \author{K.~Yoshihara\,\orcidlink{0000-0002-3656-2326}} % 12663
% \author{B.~Yu\,\orcidlink{0000-0002-2437-7289}} % 15563
% \author{C.~Z.~Yuan\,\orcidlink{0000-0002-1652-6686}} % 2088
  \author{J.~Yuan\,\orcidlink{0009-0005-0799-1630}} % 23423
  \author{Y.~Yusa\,\orcidlink{0000-0002-4001-9748}} % 2357
  \author{L.~Zani\,\orcidlink{0000-0003-4957-805X}} % 2529
  \author{F.~Zeng\,\orcidlink{0009-0003-6474-3508}} % 22043
  \author{M.~Zeyrek\,\orcidlink{0000-0002-9270-7403}} % 4023
  \author{B.~Zhang\,\orcidlink{0000-0002-5065-8762}} % 11663
% \author{J.~Z.~Zhang\,\orcidlink{0000-0001-6535-0659}} % 2349
% \author{Y.~Zhang\,\orcidlink{0000-0003-2961-2820}} % 3303
% \author{Z.~Zhang\,\orcidlink{0000-0001-6140-2044}} % 5363
% \author{J.~Zhao\,\orcidlink{0000-0001-8365-7726}} % 3343
  \author{V.~Zhilich\,\orcidlink{0000-0002-0907-5565}} % 4703
  \author{J.~S.~Zhou\,\orcidlink{0000-0002-6413-4687}} % 12463
  \author{Q.~D.~Zhou\,\orcidlink{0000-0001-5968-6359}} % 7323
% \author{X.~Y.~Zhou\,\orcidlink{0000-0002-0299-4657}} % 2380
  \author{L.~Zhu\,\orcidlink{0009-0007-1127-5818}} % 25143
% \author{V.~I.~Zhukova\,\orcidlink{0000-0002-8253-641X}} % 2387
% \author{V.~Zhulanov\,\orcidlink{0000-0002-0306-9199}} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k\,\orcidlink{0000-0003-1644-8523}} % 13403
% \author{S.~Zou\,\orcidlink{0000-0003-3377-7222}} % 19363
\collaboration{The Belle II Collaboration}


==> authors/pub084.tex <==
%%% Paper:    D+ to pi+ pi0
%%% Journal:  PhysRev
%%% Contacts: Y. Jin, A. Di Canto
%%% ====================================================================
%%% Use \input{pub084} to insert this material into your latex file.
\newcommand{\instCPPM}{Aix Marseille Universit\'{e}, CNRS/IN2P3, CPPM, 13288 Marseille, France}
\newcommand{\instYerevan}{Alikhanyan National Science Laboratory, Yerevan 0036, Armenia}
\newcommand{\instGoettingen}{II. Physikalisches Institut, Georg-August-Universit\"{a}t G\"{o}ttingen, 37073 G\"{o}ttingen, Germany}
\newcommand{\instBeihang}{Beihang University, Beijing 100191, China}
\newcommand{\instBNL}{Brookhaven National Laboratory, Upton, New York 11973, U.S.A.}
\newcommand{\instBINP}{Budker Institute of Nuclear Physics SB RAS, Novosibirsk 630090, Russian Federation}
\newcommand{\instCMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, U.S.A.}
\newcommand{\instCinvestavIPN}{Centro de Investigacion y de Estudios Avanzados del Instituto Politecnico Nacional, Mexico City 07360, Mexico}
\newcommand{\instPrague}{Faculty of Mathematics and Physics, Charles University, 121 16 Prague, Czech Republic}
\newcommand{\instChiangMai}{Chiang Mai University, Chiang Mai 50202, Thailand}
\newcommand{\instChiba}{Chiba University, Chiba 263-8522, Japan}
\newcommand{\instChonnam}{Chonnam National University, Gwangju 61186, South Korea}
\newcommand{\instChula}{Chulalongkorn University, Bangkok 10330, Thailand}
\newcommand{\instCAU}{Chung-Ang University, Seoul 06974, South Korea}
\newcommand{\instConacyt}{Consejo Nacional de Ciencia y Tecnolog\'{\i}a, Mexico City 03940, Mexico}
\newcommand{\instDESY}{Deutsches Elektronen--Synchrotron, 22607 Hamburg, Germany}
\newcommand{\instDuke}{Duke University, Durham, North Carolina 27708, U.S.A.}
\newcommand{\instITAR}{Institute of Theoretical and Applied Research (ITAR), Duy Tan University, Hanoi 100000, Vietnam}
\newcommand{\instFuJen}{Department of Physics, Fu Jen Catholic University, Taipei 24205, Taiwan}
\newcommand{\instFudan}{Key Laboratory of Nuclear Physics and Ion-beam Application (MOE) and Institute of Modern Physics, Fudan University, Shanghai 200443, China}
\newcommand{\instGifu}{Gifu University, Gifu 501-1193, Japan}
\newcommand{\instSOKENDAI}{The Graduate University for Advanced Studies (Sokendai), Tsukuba 305-0801, Japan}
\newcommand{\instMainz}{Institut f\"{u}r Kernphysik, Johannes Gutenberg-Universit\"{a}t Mainz, D-55099 Mainz, Germany}
\newcommand{\instGyeongsang}{Gyeongsang National University, Jinju 52828, South Korea}
\newcommand{\instHanyang}{Department of Physics and Institute of Natural Sciences, Hanyang University, Seoul 04763, South Korea}
\newcommand{\instHeidelberg}{Heidelberg University, 68131 Mannheim, Germany}
\newcommand{\instHNU}{Henan Normal University, Xinxiang 453007, China}
\newcommand{\instKEK}{High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instJPARC}{J-PARC Branch, KEK Theory Center, High Energy Accelerator Research Organization (KEK), Tsukuba 305-0801, Japan}
\newcommand{\instHiroshima}{Hiroshima University, Higashi-Hiroshima, Hiroshima 739-8530, Japan}
\newcommand{\instHUNNU}{Hunan Normal University, Changsha 410081, China}
\newcommand{\instFrascati}{INFN Laboratori Nazionali di Frascati, I-00044 Frascati, Italy}
\newcommand{\instNapoliINFN}{INFN Sezione di Napoli, I-80126 Napoli, Italy}
\newcommand{\instPadovaINFN}{INFN Sezione di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaINFN}{INFN Sezione di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaINFN}{INFN Sezione di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaTreINFN}{INFN Sezione di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoINFN}{INFN Sezione di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteINFN}{INFN Sezione di Trieste, I-34127 Trieste, Italy}
\newcommand{\instIISc}{Indian Institute of Science, Bengaluru 560012, India}
\newcommand{\instIISER}{Indian Institute of Science Education and Research Mohali, SAS Nagar, 140306, India}
\newcommand{\instIITBhubaneswar}{Indian Institute of Technology Bhubaneswar, Bhubaneswar 752050, India}
\newcommand{\instIITGuwahati}{Indian Institute of Technology Guwahati, Assam 781039, India}
\newcommand{\instIITHyderabad}{Indian Institute of Technology Hyderabad, Telangana 502285, India}
\newcommand{\instIITJodhpur}{Indian Institute of Technology Jodhpur, Jodhpur 342030, India}
\newcommand{\instIITMadras}{Indian Institute of Technology Madras, Chennai 600036, India}
\newcommand{\instIndiana}{Indiana University, Bloomington, Indiana 47408, U.S.A.}
\newcommand{\instIHEPRussia}{Institute for High Energy Physics, Protvino 142281, Russian Federation}
\newcommand{\instHEPHYVienna}{Institute of High Energy Physics, Vienna 1050, Austria}
\newcommand{\instIHEPChina}{Institute of High Energy Physics, Chinese Academy of Sciences, Beijing 100049, China}
\newcommand{\instIPP}{Institute of Particle Physics (Canada), Victoria, British Columbia V8W 2Y2, Canada}
\newcommand{\instIOP}{Institute of Physics, Vietnam Academy of Science and Technology (VAST), Hanoi, Vietnam}
\newcommand{\instIFIC}{Instituto de Fisica Corpuscular, Paterna 46980, Spain}
\newcommand{\instISU}{Iowa State University, Ames, Iowa 50011, U.S.A.}
\newcommand{\instJAEA}{Advanced Science Research Center, Japan Atomic Energy Agency, Naka 319-1195, Japan}
\newcommand{\instJLU}{Jilin University, Changchun 130012, China}
\newcommand{\instKarlsruhe}{Institut f\"{u}r Experimentelle Teilchenphysik, Karlsruher Institut f\"{u}r Technologie, 76131 Karlsruhe, Germany}
\newcommand{\instKitasato}{Kitasato University, Sagamihara 252-0373, Japan}
\newcommand{\instKISTI}{Korea Institute of Science and Technology Information, Daejeon 34141, South Korea}
\newcommand{\instKoreaUnivKU}{Korea University, Seoul 02841, South Korea}
\newcommand{\instKSU}{Kyoto Sangyo University, Kyoto 603-8555, Japan}
\newcommand{\instKyotoU}{Kyoto University, Kyoto 606-8501, Japan}
\newcommand{\instKyungpook}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand{\instLNNU}{Liaoning Normal University, Dalian 116029, China}
\newcommand{\instGiessen}{Justus-Liebig-Universit\"{a}t Gie\ss{}en, 35392 Gie\ss{}en, Germany}
\newcommand{\instLuther}{Luther College, Decorah, Iowa 52101, U.S.A.}
\newcommand{\instMNITJaipur}{Malaviya National Institute of Technology Jaipur, Jaipur 302017, India}
\newcommand{\instLMU}{Ludwig Maximilians University, 80539 Munich, Germany}
\newcommand{\instMcGill}{McGill University, Montr\'{e}al, Qu\'{e}bec, H3A 2T8, Canada}
\newcommand{\instMETU}{Middle East Technical University, 06531 Ankara, Turkey}
\newcommand{\instMEPhI}{Moscow Physical Engineering Institute, Moscow 115409, Russian Federation}
\newcommand{\instNagoya}{Graduate School of Science, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNagoyaKMI}{Kobayashi-Maskawa Institute, Nagoya University, Nagoya 464-8602, Japan}
\newcommand{\instNNU}{Nanjing Normal University, Nanjing 210023, China}
\newcommand{\instNankai}{Nankai University, Tianjin 300071, China}
\newcommand{\instNaraWu}{Nara Women's University, Nara 630-8506, Japan}
\newcommand{\instUNAM}{National Autonomous University of Mexico, Mexico City, Mexico}
\newcommand{\instHSE}{National Research University Higher School of Economics, Moscow 101000, Russian Federation}
\newcommand{\instNTUTaiwan}{Department of Physics, National Taiwan University, Taipei 10617, Taiwan}
\newcommand{\instKrakow}{H. Niewodniczanski Institute of Nuclear Physics, Krakow 31-342, Poland}
\newcommand{\instNiigata}{Niigata University, Niigata 950-2181, Japan}
\newcommand{\instNSU}{Novosibirsk State University, Novosibirsk 630090, Russian Federation}
\newcommand{\instOsakaMetropolitan}{Osaka Metropolitan University, Osaka 558-8585, Japan}
\newcommand{\instRCNP}{Research Center for Nuclear Physics, Osaka University, Osaka 567-0047, Japan}
\newcommand{\instPNNL}{Pacific Northwest National Laboratory, Richland, Washington 99352, U.S.A.}
\newcommand{\instPanjab}{Panjab University, Chandigarh 160014, India}
\newcommand{\instMPP}{Max-Planck-Institut f\"{u}r Physik, 80805 M\"{u}nchen, Germany}
\newcommand{\instMPGHLL}{Semiconductor Laboratory of the Max Planck Society, 81739 M\"{u}nchen, Germany}
\newcommand{\instPanjabPAU}{Punjab Agricultural University, Ludhiana 141004, India}
\newcommand{\instRIKENMSL}{Meson Science Laboratory, Cluster for Pioneering Research, RIKEN, Saitama 351-0198, Japan}
\newcommand{\instSeoul}{Seoul National University, Seoul 08826, South Korea}
\newcommand{\instShandong}{Shandong University, Jinan 250100, China}
\newcommand{\instKyiv}{Taras Shevchenko National University of Kiev, Kiev, Ukraine}
\newcommand{\instSPU}{Showa Pharmaceutical University, Tokyo 194-8543, Japan}
\newcommand{\instSoochow}{Soochow University, Suzhou 215006, China}
\newcommand{\instSoongsil}{Department of Physics and Origin of Matter and Evolution of Galaxy (OMEG) Institute, Soongsil University, Seoul 06978, South Korea}
\newcommand{\instSEU}{Southeast University, Nanjing 211189, China}
\newcommand{\instLjubljanaJSI}{J. Stefan Institute, 1000 Ljubljana, Slovenia}
\newcommand{\instSKKU}{Sungkyunkwan University, Suwon 16419, South Korea}
\newcommand{\instTata}{Tata Institute of Fundamental Research, Mumbai 400005, India}
\newcommand{\instTUM}{Department of Physics, Technische Universit\"{a}t M\"{u}nchen, 85748 Garching, Germany}
\newcommand{\instTelAviv}{School of Physics and Astronomy, Tel Aviv University, Tel Aviv 69978, Israel}
\newcommand{\instToho}{Toho University, Funabashi 274-8510, Japan}
\newcommand{\instTitech}{Tokyo Institute of Technology, Tokyo 152-8550, Japan}
\newcommand{\instTokyoMetropolitan}{Tokyo Metropolitan University, Tokyo 192-0397, Japan}
\newcommand{\instUAS}{Universidad Autonoma de Sinaloa, Sinaloa 80000, Mexico}
\newcommand{\instNapoliUNIV}{Dipartimento di Scienze Fisiche, Universit\`{a} di Napoli Federico II, I-80126 Napoli, Italy}
\newcommand{\instPadovaUNIV}{Dipartimento di Fisica e Astronomia, Universit\`{a} di Padova, I-35131 Padova, Italy}
\newcommand{\instPerugiaUNIV}{Dipartimento di Fisica, Universit\`{a} di Perugia, I-06123 Perugia, Italy}
\newcommand{\instPisaUNIV}{Dipartimento di Fisica, Universit\`{a} di Pisa, I-56127 Pisa, Italy}
\newcommand{\instRomaTreUNIV}{Dipartimento di Matematica e Fisica, Universit\`{a} di Roma Tre, I-00146 Roma, Italy}
\newcommand{\instTorinoUNIV}{Dipartimento di Fisica, Universit\`{a} di Torino, I-10125 Torino, Italy}
\newcommand{\instTriesteUNIV}{Dipartimento di Fisica, Universit\`{a} di Trieste, I-34127 Trieste, Italy}
\newcommand{\instIJCLab}{Universit\'{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand{\instIPHC}{Universit\'{e} de Strasbourg, CNRS, IPHC, UMR 7178, 67037 Strasbourg, France}
\newcommand{\instAdelaide}{Department of Physics, University of Adelaide, Adelaide, South Australia 5005, Australia}
\newcommand{\instUofA}{University of Alberta, Edmonton, Alberta, T6G 2E1, Canada}
\newcommand{\instBonn}{University of Bonn, 53115 Bonn, Germany}
\newcommand{\instUBC}{University of British Columbia, Vancouver, British Columbia, V6T 1Z1, Canada}
\newcommand{\instCincinnati}{University of Cincinnati, Cincinnati, Ohio 45221, U.S.A.}
\newcommand{\instFlorida}{University of Florida, Gainesville, Florida 32611, U.S.A.}
\newcommand{\instHamburg}{University of Hamburg, 20148 Hamburg, Germany}
\newcommand{\instHawaii}{University of Hawaii, Honolulu, Hawaii 96822, U.S.A.}
\newcommand{\instLjubljanaUniLJ}{Faculty of Mathematics and Physics, University of Ljubljana, 1000 Ljubljana, Slovenia}
\newcommand{\instLouisville}{University of Louisville, Louisville, Kentucky 40292, U.S.A.}
\newcommand{\instMalaya}{National Centre for Particle Physics, University of Malaya, 50603 Kuala Lumpur, Malaysia}
\newcommand{\instManitoba}{University of Manitoba, Winnipeg, Manitoba, R3T 2N2, Canada}
\newcommand{\instLjubljanaUM}{Faculty of Chemistry and Chemical Engineering, University of Maribor, 2000 Maribor, Slovenia}
\newcommand{\instMelbourne}{School of Physics, University of Melbourne, Victoria 3010, Australia}
\newcommand{\instMississippi}{University of Mississippi, University, Mississippi 38677, U.S.A.}
\newcommand{\instUOM}{University of Miyazaki, Miyazaki 889-2192, Japan}
\newcommand{\instNovaGorica}{University of Nova Gorica, 5000 Nova Gorica, Slovenia}
\newcommand{\instUPES}{University of Petroleum and Energy Studies, Dehradun 248007, India}
\newcommand{\instPittsburgh}{University of Pittsburgh, Pittsburgh, Pennsylvania 15260, U.S.A.}
\newcommand{\instUSTC}{Department of Modern Physics and State Key Laboratory of Particle Detection and Electronics, University of Science and Technology of China, Hefei 230026, China}
\newcommand{\instSAlabama}{University of South Alabama, Mobile, Alabama 36688, U.S.A.}
\newcommand{\instSCarolina}{University of South Carolina, Columbia, South Carolina 29208, U.S.A.}
\newcommand{\instSydney}{School of Physics, University of Sydney, New South Wales 2006, Australia}
\newcommand{\instTabuk}{Department of Physics, Faculty of Science, University of Tabuk, Tabuk 71451, Saudi Arabia}
\newcommand{\instUTokyo}{Department of Physics, University of Tokyo, Tokyo 113-0033, Japan}
\newcommand{\instEri}{Earthquake Research Institute, University of Tokyo, Tokyo 113-0032, Japan}
\newcommand{\instIPMU}{Kavli Institute for the Physics and Mathematics of the Universe (WPI), University of Tokyo, Kashiwa 277-8583, Japan}
\newcommand{\instVictoria}{University of Victoria, Victoria, British Columbia, V8W 3P6, Canada}
\newcommand{\instUppsala}{Uppsala University, SE-751 05 Uppsala, Sweden}
\newcommand{\instVPI}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, U.S.A.}
\newcommand{\instWayneState}{Wayne State University, Detroit, Michigan 48202, U.S.A.}
\newcommand{\instXavier}{St. Francis Xavier University, Antigonish, Nova Scotia, B2G 2W5, Canada}
\newcommand{\instXJTU}{Xi'an Jiaotong University, Xi'an 710049, China}
\newcommand{\instYamagata}{Yamagata University, Yamagata 990-8560, Japan}
\newcommand{\instYonsei}{Yonsei University, Seoul 03722, South Korea}
\newcommand{\instTYL}{Toshiko Yuasa Laboratory, Tsukuba 305-0801, Japan}
\newcommand{\instZZU}{Zhengzhou University, Zhengzhou 450001, China}
\affiliation{\instCPPM}
\affiliation{\instYerevan}
\affiliation{\instGoettingen}
\affiliation{\instBeihang}
\affiliation{\instBNL}
\affiliation{\instBINP}
\affiliation{\instCMU}
\affiliation{\instCinvestavIPN}
\affiliation{\instPrague}
\affiliation{\instChiangMai}
%%%\affiliation{\instChiba}
\affiliation{\instChonnam}
%%%\affiliation{\instChula}
\affiliation{\instCAU}
\affiliation{\instConacyt}
\affiliation{\instDESY}
\affiliation{\instDuke}
\affiliation{\instITAR}
\affiliation{\instFuJen}
\affiliation{\instFudan}
\affiliation{\instGifu}
\affiliation{\instSOKENDAI}
\affiliation{\instMainz}
\affiliation{\instGyeongsang}
\affiliation{\instHanyang}
%%%\affiliation{\instHeidelberg}
\affiliation{\instHNU}
\affiliation{\instKEK}
\affiliation{\instJPARC}
%%%\affiliation{\instHiroshima}
\affiliation{\instHUNNU}
\affiliation{\instFrascati}
\affiliation{\instNapoliINFN}
\affiliation{\instPadovaINFN}
\affiliation{\instPerugiaINFN}
\affiliation{\instPisaINFN}
\affiliation{\instRomaTreINFN}
\affiliation{\instTorinoINFN}
\affiliation{\instTriesteINFN}
\affiliation{\instIISc}
\affiliation{\instIISER}
\affiliation{\instIITBhubaneswar}
\affiliation{\instIITGuwahati}
\affiliation{\instIITHyderabad}
%%%\affiliation{\instIITJodhpur}
\affiliation{\instIITMadras}
\affiliation{\instIndiana}
\affiliation{\instIHEPRussia}
\affiliation{\instHEPHYVienna}
\affiliation{\instIHEPChina}
\affiliation{\instIPP}
\affiliation{\instIOP}
\affiliation{\instIFIC}
\affiliation{\instISU}
\affiliation{\instJAEA}
\affiliation{\instJLU}
\affiliation{\instKarlsruhe}
\affiliation{\instKitasato}
\affiliation{\instKISTI}
\affiliation{\instKoreaUnivKU}
%%%\affiliation{\instKSU}
\affiliation{\instKyotoU}
\affiliation{\instKyungpook}
\affiliation{\instLNNU}
\affiliation{\instGiessen}
\affiliation{\instLuther}
\affiliation{\instMNITJaipur}
\affiliation{\instLMU}
\affiliation{\instMcGill}
\affiliation{\instMETU}
%%%\affiliation{\instMEPhI}
\affiliation{\instNagoya}
\affiliation{\instNagoyaKMI}
\affiliation{\instNNU}
\affiliation{\instNankai}
\affiliation{\instNaraWu}
%%%\affiliation{\instUNAM}
\affiliation{\instHSE}
\affiliation{\instNTUTaiwan}
\affiliation{\instKrakow}
\affiliation{\instNiigata}
\affiliation{\instNSU}
\affiliation{\instOsakaMetropolitan}
\affiliation{\instRCNP}
\affiliation{\instPNNL}
\affiliation{\instPanjab}
\affiliation{\instMPP}
%%%\affiliation{\instMPGHLL}
\affiliation{\instPanjabPAU}
\affiliation{\instRIKENMSL}
%%%\affiliation{\instSeoul}
\affiliation{\instShandong}
\affiliation{\instKyiv}
\affiliation{\instSPU}
\affiliation{\instSoochow}
\affiliation{\instSoongsil}
\affiliation{\instSEU}
\affiliation{\instLjubljanaJSI}
\affiliation{\instSKKU}
\affiliation{\instTata}
\affiliation{\instTUM}
\affiliation{\instTelAviv}
%%%\affiliation{\instToho}
\affiliation{\instTitech}
%%%\affiliation{\instTokyoMetropolitan}
\affiliation{\instUAS}
\affiliation{\instNapoliUNIV}
\affiliation{\instPadovaUNIV}
\affiliation{\instPerugiaUNIV}
\affiliation{\instPisaUNIV}
\affiliation{\instRomaTreUNIV}
\affiliation{\instTorinoUNIV}
\affiliation{\instTriesteUNIV}
\affiliation{\instIJCLab}
\affiliation{\instIPHC}
%%%\affiliation{\instAdelaide}
\affiliation{\instUofA}
\affiliation{\instBonn}
\affiliation{\instUBC}
\affiliation{\instCincinnati}
\affiliation{\instFlorida}
\affiliation{\instHamburg}
\affiliation{\instHawaii}
\affiliation{\instLjubljanaUniLJ}
\affiliation{\instLouisville}
%%%\affiliation{\instMalaya}
\affiliation{\instManitoba}
\affiliation{\instLjubljanaUM}
\affiliation{\instMelbourne}
\affiliation{\instMississippi}
%%%\affiliation{\instUOM}
%%%\affiliation{\instNovaGorica}
\affiliation{\instUPES}
\affiliation{\instPittsburgh}
\affiliation{\instUSTC}
\affiliation{\instSAlabama}
%%%\affiliation{\instSCarolina}
\affiliation{\instSydney}
\affiliation{\instTabuk}
\affiliation{\instUTokyo}
\affiliation{\instEri}
\affiliation{\instIPMU}
\affiliation{\instVictoria}
\affiliation{\instUppsala}
\affiliation{\instVPI}
\affiliation{\instWayneState}
\affiliation{\instXavier}
\affiliation{\instXJTU}
\affiliation{\instYamagata}
\affiliation{\instYonsei}
\affiliation{\instTYL}
%%%\affiliation{\instZZU}
  \author{I.~Adachi}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2590
% \author{K.~Adamczyk}\affiliation{\instKrakow} % 2239
  \author{L.~Aggarwal}\affiliation{\instPanjab} % 10083
% \author{P.~Ahlburg}\affiliation{\instBonn} % 2367
  \author{H.~Ahmed}\affiliation{\instXavier} % 11323
% \author{J.~K.~Ahn}\affiliation{\instKoreaUnivKU} % 7423
% \author{Y.~Ahn}\affiliation{\instKoreaUnivKU} % 14363
  \author{H.~Aihara}\affiliation{\instUTokyo} % 2223
  \author{N.~Akopov}\affiliation{\instYerevan} % 9443
  \author{S.~Alghamdi}\affiliation{\instTabuk} % 27804
  \author{M.~Alhakami}\affiliation{\instTabuk} % 28103
  \author{A.~Aloisio}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2194
% \author{N.~Althubiti}\affiliation{\instTabuk} % 21524
  \author{K.~Amos}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 27583
% \author{L.~Andricek}\affiliation{\instMPGHLL} % 2098
  \author{M.~Angelsmark}\affiliation{\instBonn} % 13963
  \author{N.~Anh~Ky}\affiliation{\instIOP} % 2218
  \author{C.~Antonioli}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 20583
  \author{D.~M.~Asner}\affiliation{\instHawaii} % 4684
  \author{H.~Atmacan}\affiliation{\instCincinnati} % 2538
% \author{V.~Aulchenko}\affiliation{\instBINP}\affiliation{\instNSU} % 8183
% \author{T.~Aushev}\affiliation{\instHSE} % 3747
  \author{V.~Aushev}\affiliation{\instKyiv} % 2155
  \author{M.~Aversano}\affiliation{\instNagoya} % 7363
  \author{R.~Ayad}\affiliation{\instTabuk} % 3766
% \author{T.~Aziz}\affiliation{\instTata} % 3523
  \author{V.~Babu}\affiliation{\instIPHC} % 5623
% \author{S.~Bacher}\affiliation{\instKrakow} % 2258
  \author{H.~Bae}\affiliation{\instKEK} % 10863
  \author{N.~K.~Baghel}\affiliation{\instLouisville} % 21505
% \author{S.~Bahinipati}\affiliation{\instIITBhubaneswar} % 2332
% \author{A.~M.~Bakich}\affiliation{\instSydney} % 2115
  \author{P.~Bambade}\affiliation{\instIJCLab} % 3003
  \author{Sw.~Banerjee}\affiliation{\instLouisville} % 8603
  \author{S.~Bansal}\affiliation{\instPanjab} % 5163
  \author{M.~Barrett}\affiliation{\instKEK} % 2180
  \author{M.~Bartl}\affiliation{\instMPP} % 26483
% \author{G.~Batignani}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 6643
  \author{J.~Baudot}\affiliation{\instIPHC} % 2562
% \author{M.~Bauer}\affiliation{\instKarlsruhe} % 9863
  \author{A.~Baur}\affiliation{\instDESY} % 5683
  \author{A.~Beaubien}\affiliation{\instVictoria} % 6683
  \author{F.~Becherer}\affiliation{\instDESY} % 21623
  \author{J.~Becker}\affiliation{\instKarlsruhe} % 5403
% \author{P.~K.~Behera}\affiliation{\instIITMadras} % 4204
  \author{J.~V.~Bennett}\affiliation{\instMississippi} % 2454
% \author{E.~Bernieri}\affiliation{\instRomaTreINFN} % 4483
  \author{F.~U.~Bernlochner}\affiliation{\instBonn} % 2282
  \author{V.~Bertacchi}\affiliation{\instBonn} % 2212
  \author{M.~Bertemes}\affiliation{\instHEPHYVienna} % 2595
  \author{E.~Bertholet}\affiliation{\instTelAviv} % 13163
  \author{M.~Bessner}\affiliation{\instHawaii} % 3783
% \author{D.~Z.~Besson}\affiliation{\instMEPhI} % 3585
  \author{S.~Bettarini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2350
  \author{V.~Bhardwaj}\affiliation{\instIISER} % 2228
  \author{B.~Bhuyan}\affiliation{\instIITGuwahati} % 2097
  \author{F.~Bianchi}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2564
% \author{L.~Bierwirth}\affiliation{\instTUM} % 11723
% \author{T.~Bilka}\affiliation{\instDESY} % 2484
% \author{S.~Bilokin}\affiliation{\instLMU} % 3623
  \author{D.~Biswas}\affiliation{\instLouisville} % 8703
% \author{T.~Bloomfield}\affiliation{\instKEK} % 2418
  \author{A.~Bobrov}\affiliation{\instBINP}\affiliation{\instNSU} % 2294
  \author{D.~Bodrov}\affiliation{\instSoochow}\affiliation{\instHSE} % 9643
% \author{A.~Bolz}\affiliation{\instDESY} % 15403
  \author{A.~Bondar}\affiliation{\instBINP}\affiliation{\instNSU} % 4643
  \author{G.~Bonvicini}\affiliation{\instWayneState} % 2095
  \author{J.~Borah}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 7083
  \author{A.~Boschetti}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 17683
  \author{A.~Bozek}\affiliation{\instKrakow} % 2303
  \author{M.~Bra\v{c}ko}\affiliation{\instLjubljanaJSI}\affiliation{\instLjubljanaUM} % 2425
  \author{P.~Branchini}\affiliation{\instRomaTreINFN} % 2577
% \author{N.~Brenny}\affiliation{\instISU} % 19943
  \author{R.~A.~Briere}\affiliation{\instCMU} % 2584
  \author{T.~E.~Browder}\affiliation{\instHawaii} % 2560
% \author{Y.~Buch}\affiliation{\instGoettingen} % 17323
  \author{A.~Budano}\affiliation{\instRomaTreINFN} % 2171
  \author{S.~Bussino}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 5384
% \author{A.~Calcaterra}\affiliation{\instFrascati} % 19163
% \author{A.~Caldwell}\affiliation{\instMPP} % 2608
  \author{Q.~Campagna}\affiliation{\instMississippi} % 21563
  \author{M.~Campajola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 5223
  \author{L.~Cao}\affiliation{\instFudan} % 2099
  \author{G.~Casarosa}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2491
  \author{C.~Cecchi}\affiliation{\instPerugiaUNIV}\affiliation{\instPerugiaINFN} % 2433
% \author{J.~Cerasoli}\affiliation{\instIPHC} % 20746
  \author{M.-C.~Chang}\affiliation{\instFuJen} % 2827
% \author{P.~Chang}\affiliation{\instNTUTaiwan} % 2542
% \author{R.~Cheaib}\affiliation{\instDESY} % 2208
  \author{P.~Cheema}\affiliation{\instSydney} % 15264
% \author{V.~Chekelian}\affiliation{\instMPP} % 2167
% \author{C.~Chen}\affiliation{\instISU} % 12803
  \author{L.~Chen}\affiliation{\instNNU} % 17363
% \author{Y.-T.~Chen}\affiliation{\instNTUTaiwan} % 2884
  \author{B.~G.~Cheon}\affiliation{\instHanyang} % 2173
% \author{C.~Cheshta}\affiliation{\instTata} % 25483
  \author{K.~Chilikin}\affiliation{\instBINP} % 2308
  \author{J.~Chin}\affiliation{\instCincinnati} % 20283
  \author{K.~Chirapatpimol}\affiliation{\instChiangMai} % 10803
  \author{H.-E.~Cho}\affiliation{\instHanyang} % 2182
  \author{K.~Cho}\affiliation{\instKISTI} % 2516
  \author{S.-J.~Cho}\affiliation{\instYonsei} % 2723
  \author{S.-K.~Choi}\affiliation{\instCAU} % 2364
  \author{S.~Choudhury}\affiliation{\instISU} % 2206
% \author{K.~Chu}\affiliation{\instMcGill} % 5203
% \author{D.~Cinabro}\affiliation{\instWayneState} % 2092
% \author{J.~Cochran}\affiliation{\instISU} % 12604
  \author{I.~Consigny}\affiliation{\instCPPM} % 23903
  \author{L.~Corona}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 3944
% \author{L.~M.~Cremaldi}\affiliation{\instMississippi} % 2276
  \author{J.~X.~Cui}\affiliation{\instSEU} % 8863
% \author{T.~Czank}\affiliation{\instTokyoMetropolitan} % 2254
  \author{S.~Das}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 9163
% \author{F.~Dattola}\affiliation{\instDESY} % 3745
  \author{E.~De~La~Cruz-Burelo}\affiliation{\instCinvestavIPN} % 2359
  \author{S.~A.~De~La~Motte}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2128
% \author{G.~de~Marino}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 8364
% \author{G.~De~Nardo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2459
% \author{M.~De~Nuccio}\affiliation{\instUBC} % 2610
  \author{G.~De~Pietro}\affiliation{\instKarlsruhe} % 2528
  \author{R.~de~Sangro}\affiliation{\instFrascati} % 2524
% \author{B.~Deschamps}\affiliation{\instBonn} % 2671
  \author{M.~Destefanis}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2594
% \author{S.~Dey}\affiliation{\instKEK} % 5023
% \author{A.~De~Yta-Hernandez}\affiliation{\instCinvestavIPN} % 2104
% \author{R.~Dhamija}\affiliation{\instIITHyderabad} % 9465
  \author{A.~Di~Canto}\affiliation{\instBNL} % 10963
% \author{F.~Di~Capua}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2065
% \author{J.~Dingfelder}\affiliation{\instBonn} % 2151
  \author{Z.~Dole\v{z}al}\affiliation{\instPrague} % 2319
  \author{I.~Dom\'{\i}nguez~Jim\'{e}nez}\affiliation{\instUAS} % 2191
  \author{T.~V.~Dong}\affiliation{\instITAR} % 2215
  \author{X.~Dong}\affiliation{\instDESY} % 17343
  \author{M.~Dorigo}\affiliation{\instTriesteINFN} % 12543
% \author{D.~Dorner}\affiliation{\instHEPHYVienna} % 13564
% \author{K.~Dort}\affiliation{\instGiessen} % 5583
% \author{D.~Dossett}\affiliation{\instMelbourne} % 2574
% \author{S.~Dreyer}\affiliation{\instDESY} % 12823
% \author{S.~Dubey}\affiliation{\instHawaii} % 11063
% \author{S.~Duell}\affiliation{\instBonn} % 2344
  \author{K.~Dugic}\affiliation{\instMPP} % 11103
  \author{G.~Dujany}\affiliation{\instIPHC} % 9703
  \author{P.~Ecker}\affiliation{\instKarlsruhe} % 5563
% \author{M.~Eliachevitch}\affiliation{\instBonn} % 2725
  \author{D.~Epifanov}\affiliation{\instBINP}\affiliation{\instNSU} % 2551
  \author{J.~Eppelt}\affiliation{\instKarlsruhe} % 19723
% \author{Y.~Fan}\affiliation{\instDESY} % 21303
  \author{R.~Farkas}\affiliation{\instBonn} % 12843
  \author{P.~Feichtinger}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 9843
  \author{T.~Ferber}\affiliation{\instKarlsruhe} % 2482
% \author{D.~Ferlewicz}\affiliation{\instMelbourne} % 2073
  \author{T.~Fillinger}\affiliation{\instKEK} % 9803
  \author{C.~Finck}\affiliation{\instIPHC} % 15803
  \author{G.~Finocchiaro}\affiliation{\instFrascati} % 2400
% \author{P.~Fischer}\affiliation{\instHeidelberg} % 2141
% \author{K.~Flood}\affiliation{\instHawaii} % 12103
% \author{A.~Fodor}\affiliation{\instMcGill} % 2312
  \author{F.~Forti}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2432
  \author{A.~Frey}\affiliation{\instGoettingen} % 2150
% \author{M.~Friedl}\affiliation{\instHEPHYVienna} % 2442
  \author{B.~G.~Fulsom}\affiliation{\instPNNL} % 2563
  \author{A.~Gabrielli}\affiliation{\instPisaINFN} % 13523
% \author{N.~Gabyshev}\affiliation{\instBINP}\affiliation{\instNSU} % 2510
  \author{A.~Gale}\affiliation{\instCincinnati} % 20263
  \author{E.~Ganiev}\affiliation{\instLjubljanaUniLJ} % 4623
  \author{M.~Garcia-Hernandez}\affiliation{\instKEK} % 4823
  \author{R.~Garg}\affiliation{\instCMU} % 2213
% \author{A.~Garmash}\affiliation{\instBINP}\affiliation{\instNSU} % 2161
% \author{L.~G\"artner}\affiliation{\instLMU} % 21783
  \author{G.~Gaudino}\affiliation{\instNapoliINFN} % 16563
  \author{V.~Gaur}\affiliation{\instUPES} % 2413
  \author{V.~Gautam}\affiliation{\instIITBhubaneswar} % 22223
  \author{A.~Gaz}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2181
  \author{A.~Gellrich}\affiliation{\instDESY} % 2480
% \author{G.~Ghevondyan}\affiliation{\instYerevan} % 9445
  \author{D.~Ghosh}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 11923
  \author{H.~Ghumaryan}\affiliation{\instYerevan} % 19543
  \author{G.~Giakoustidis}\affiliation{\instBonn} % 13723
  \author{R.~Giordano}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2103
  \author{A.~Giri}\affiliation{\instIITHyderabad} % 2106
  \author{P.~Gironella~Gironell}\affiliation{\instIPHC} % 25443
% \author{A.~Glazov}\affiliation{\instDESY} % 2473
  \author{B.~Gobbo}\affiliation{\instTriesteINFN} % 2109
  \author{R.~Godang}\affiliation{\instSAlabama} % 2449
  \author{O.~Gogota}\affiliation{\instKyiv} % 2334
  \author{P.~Goldenzweig}\affiliation{\instKarlsruhe} % 2345
% \author{B.~Golob}\affiliation{\instNovaGorica}\affiliation{\instLjubljanaJSI} % 3703
% \author{G.~Gong}\affiliation{\instUSTC} % 2727
% \author{P.~Grace}\affiliation{\instAdelaide} % 9563
  \author{W.~Gradl}\affiliation{\instMainz} % 2570
% \author{M.~Graf-Schreiber}\affiliation{\instDESY} % 2730
% \author{T.~Grammatico}\affiliation{\instVictoria} % 20623
% \author{S.~Granderath}\affiliation{\instBonn} % 8383
  \author{E.~Graziani}\affiliation{\instRomaTreINFN} % 2342
  \author{D.~Greenwald}\affiliation{\instTUM} % 2686
% \author{T.~Gu}\affiliation{\instPittsburgh} % 14283
  \author{Y.~Guan}\affiliation{\instCincinnati} % 2514
  \author{K.~Gudkova}\affiliation{\instBINP}\affiliation{\instNSU} % 10504
  \author{I.~Haide}\affiliation{\instKarlsruhe} % 14824
% \author{H.~Haigh}\affiliation{\instHEPHYVienna} % 16744
% \author{S.~Halder}\affiliation{\instTata} % 4743
% \author{Y.~Han}\affiliation{\instHawaii} % 19663
% \author{K.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2462
% \author{T.~Hara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2523
% \author{C.~Harris}\affiliation{\instAdelaide} % 21383
% \author{K.~Hayasaka}\affiliation{\instNiigata} % 2330
  \author{H.~Hayashii}\affiliation{\instNaraWu} % 2455
  \author{S.~Hazra}\affiliation{\instMPP} % 7663
  \author{C.~Hearty}\affiliation{\instUBC}\affiliation{\instIPP} % 2450
  \author{M.~T.~Hedges}\affiliation{\instBonn} % 2265
  \author{A.~Heidelbach}\affiliation{\instKarlsruhe} % 16923
  \author{G.~Heine}\affiliation{\instKarlsruhe} % 23863
  \author{I.~Heredia~de~la~Cruz}\affiliation{\instCinvestavIPN}\affiliation{\instConacyt} % 2559
  \author{M.~Hern\'{a}ndez~Villanueva}\affiliation{\instBNL} % 2466
  \author{T.~Higuchi}\affiliation{\instIPMU} % 2485
% \author{H.~Hirata}\affiliation{\instNagoya} % 2070
  \author{M.~Hoek}\affiliation{\instMainz} % 2101
  \author{M.~Hohmann}\affiliation{\instDESY} % 2077
  \author{R.~Hoppe}\affiliation{\instDESY} % 23383
  \author{P.~Horak}\affiliation{\instVictoria} % 13583
% \author{T.~Hotta}\affiliation{\instRCNP} % 2084
  \author{C.-L.~Hsu}\affiliation{\instSydney} % 2299
% \author{A.~Huang}\affiliation{\instSydney} % 14223
% \author{K.~Huang}\affiliation{\instNTUTaiwan} % 2389
  \author{T.~Humair}\affiliation{\instDESY} % 10643
  \author{T.~Iijima}\affiliation{\instNagoya}\affiliation{\instNagoyaKMI}\affiliation{\instKEK} % 2446
  \author{K.~Inami}\affiliation{\instNagoya}\affiliation{\instKEK} % 2323
  \author{G.~Inguglia}\affiliation{\instHEPHYVienna} % 2500
  \author{N.~Ipsita}\affiliation{\instIITHyderabad} % 12223
% \author{C.~Irmler}\affiliation{\instHEPHYVienna} % 2186
  \author{A.~Ishikawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2281
  \author{R.~Itoh}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2487
  \author{M.~Iwasaki}\affiliation{\instOsakaMetropolitan} % 2360
% \author{Y.~Iwasaki}\affiliation{\instKEK} % 2229
% \author{S.~Iwata}\affiliation{\instTokyoMetropolitan} % 4323
% \author{P.~Jackson}\affiliation{\instAdelaide} % 2255
  \author{D.~Jacobi}\affiliation{\instBonn} % 15123
  \author{W.~W.~Jacobs}\affiliation{\instIndiana} % 2322
  \author{D.~E.~Jaffe}\affiliation{\instBNL} % 3663
  \author{E.-J.~Jang}\affiliation{\instGyeongsang} % 6744
  \author{Q.~P.~Ji}\affiliation{\instHNU} % 16243
% \author{X.~B.~Ji}\affiliation{\instIHEPChina} % 2558
  \author{S.~Jia}\affiliation{\instSEU} % 2457
  \author{Y.~Jin}\affiliation{\instBNL} % 2105
  \author{A.~Johnson}\affiliation{\instIITMadras} % 16143
  \author{K.~K.~Joo}\affiliation{\instChonnam} % 4224
% \author{H.~Junkerkalefeld}\affiliation{\instBonn} % 12963
% \author{I.~Kadenko}\affiliation{\instKyiv} % 3843
% \author{H.~Kakuno}\affiliation{\instTokyoMetropolitan} % 2391
% \author{M.~Kaleta}\affiliation{\instKrakow} % 5603
% \author{D.~Kalita}\affiliation{\instIITGuwahati} % 2220
% \author{A.~B.~Kaliyar}\affiliation{\instHEPHYVienna} % 7344
  \author{J.~Kandra}\affiliation{\instPadovaINFN} % 2541
  \author{K.~H.~Kang}\affiliation{\instKyungpook} % 2283
% \author{S.~Kang}\affiliation{\instISU} % 12683
  \author{G.~Karyan}\affiliation{\instYerevan} % 2550
% \author{H.~Kawai}\affiliation{\instChiba} % 4344
  \author{T.~Kawasaki}\affiliation{\instKitasato} % 4363
  \author{F.~Keil}\affiliation{\instMainz} % 19523
  \author{C.~Ketter}\affiliation{\instHawaii} % 2236
% \author{M.~Khan}\affiliation{\instBonn} % 15644
  \author{C.~Kiesling}\affiliation{\instMPP} % 2168
% \author{C.~Kim}\affiliation{\instYonsei} % 20503
  \author{C.-H.~Kim}\affiliation{\instHanyang} % 2358
  \author{D.~Y.~Kim}\affiliation{\instSoongsil} % 2315
  \author{J.-Y.~Kim}\affiliation{\instYonsei} % 20223
  \author{K.-H.~Kim}\affiliation{\instSKKU} % 2118
% \author{S.~K.~Kim}\affiliation{\instSeoul} % 3823
% \author{Y.~J.~Kim}\affiliation{\instKoreaUnivKU} % 2403
  \author{Y.-K.~Kim}\affiliation{\instYonsei} % 2379
  \author{H.~Kindo}\affiliation{\instVPI}\affiliation{\instKEK} % 2195
  \author{K.~Kinoshita}\affiliation{\instCincinnati} % 2318
  \author{P.~Kody\v{s}}\affiliation{\instPrague} % 2407
  \author{T.~Koga}\affiliation{\instKEK} % 6963
  \author{S.~Kohani}\affiliation{\instHawaii} % 9143
  \author{K.~Kojima}\affiliation{\instNagoya} % 6363
% \author{T.~Konno}\affiliation{\instKitasato} % 2490
% \author{H.~Korandla}\affiliation{\instHawaii} % 18783
  \author{A.~Korobov}\affiliation{\instBINP}\affiliation{\instNSU} % 4185
  \author{S.~Korpar}\affiliation{\instLjubljanaJSI}\affiliation{\instLjubljanaUM} % 2475
% \author{E.~Kou}\affiliation{\instIJCLab} % 3765
  \author{E.~Kovalenko}\affiliation{\instBINP}\affiliation{\instNSU} % 3884
  \author{R.~Kowalewski}\affiliation{\instVictoria} % 2293
% \author{T.~M.~G.~Kraetzschmar}\affiliation{\instMPP} % 7543
  \author{P.~Kri\v{z}an}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2474
% \author{R.~Kroeger}\affiliation{\instMississippi} % 2242
  \author{P.~Krokovny}\affiliation{\instBINP}\affiliation{\instNSU} % 2575
% \author{W.~Kuehn}\affiliation{\instGiessen} % 2534
% \author{T.~Kuhr}\affiliation{\instLMU} % 2486
  \author{Y.~Kulii}\affiliation{\instLMU} % 9823
% \author{D.~Kumar}\affiliation{\instKrakow} % 7223
% \author{J.~Kumar}\affiliation{\instIITJodhpur} % 6464
% \author{M.~Kumar}\affiliation{\instIISER} % 2744
  \author{R.~Kumar}\affiliation{\instPanjabPAU} % 2189
  \author{K.~Kumara}\affiliation{\instMississippi} % 2257
% \author{T.~Kumita}\affiliation{\instTokyoMetropolitan} % 4083
  \author{T.~Kunigo}\affiliation{\instKEK} % 10104
% \author{A.~Kusudo}\affiliation{\instNaraWu} % 14623
  \author{A.~Kuzmin}\affiliation{\instBINP}\affiliation{\instNSU} % 2520
% \author{P.~Kvasni\v{c}ka}\affiliation{\instPrague} % 2184
  \author{Y.-J.~Kwon}\affiliation{\instYonsei} % 2231
% \author{S.~Lacaprara}\affiliation{\instPadovaINFN} % 2447
% \author{Y.-T.~Lai}\affiliation{\instKEK} % 2066
  \author{K.~Lalwani}\affiliation{\instMNITJaipur} % 2142
  \author{T.~Lam}\affiliation{\instVPI} % 2729
  \author{L.~Lanceri}\affiliation{\instTriesteINFN} % 2540
  \author{J.~S.~Lange}\affiliation{\instGiessen} % 2277
  \author{T.~S.~Lau}\affiliation{\instKEK} % 19803
  \author{M.~Laurenza}\affiliation{\instUppsala} % 10223
% \author{K.~Lautenbach}\affiliation{\instCPPM} % 2102
% \author{P.~J.~Laycock}\affiliation{\instBNL} % 7683
  \author{R.~Leboucher}\affiliation{\instUBC} % 14083
  \author{F.~R.~Le~Diberder}\affiliation{\instIJCLab} % 3267
  \author{M.~J.~Lee}\affiliation{\instSKKU} % 21803
% \author{P.~Leitl}\affiliation{\instMPP} % 2414
  \author{C.~Lemettais}\affiliation{\instCPPM} % 22704
  \author{P.~Leo}\affiliation{\instDESY}\affiliation{\instHamburg} % 19823
% \author{D.~Levit}\affiliation{\instKEK} % 2507
  \author{P.~M.~Lewis}\affiliation{\instHawaii} % 2582
  \author{C.~Li}\affiliation{\instLNNU} % 2325
  \author{H.-J.~Li}\affiliation{\instHNU} % 4943
  \author{L.~K.~Li}\affiliation{\instHUNNU} % 3263
% \author{Q.~M.~Li}\affiliation{\instIHEPChina} % 22943
  \author{S.~X.~Li}\affiliation{\instFudan} % 2377
  \author{W.~Z.~Li}\affiliation{\instBeihang} % 19703
  \author{Y.~Li}\affiliation{\instFudan} % 8083
  \author{Y.~B.~Li}\affiliation{\instXJTU} % 2573
  \author{Y.~P.~Liao}\affiliation{\instIHEPChina} % 24303
  \author{J.~Libby}\affiliation{\instIITMadras} % 2262
  \author{J.~Lin}\affiliation{\instNTUTaiwan} % 2401
  \author{S.~Lin}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 17223
% \author{Z.~Liptak}\affiliation{\instHiroshima} % 3565
% \author{V.~Lisovskyi}\affiliation{\instCPPM} % 26584
% \author{A.~Little}\affiliation{\instSydney} % 23803
  \author{M.~H.~Liu}\affiliation{\instJLU} % 15244
  \author{Q.~Y.~Liu}\affiliation{\instHawaii} % 7045
  \author{Y.~Liu}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 16223
  \author{Z.~Liu}\affiliation{\instShandong} % 11303
% \author{Z.~A.~Liu}\affiliation{\instIHEPChina} % 3283
  \author{D.~Liventsev}\affiliation{\instWayneState}\affiliation{\instKEK} % 2578
  \author{S.~Longo}\affiliation{\instManitoba} % 2396
% \author{G.~Lopez-Castro}\affiliation{\instCinvestavIPN} % 4245
  \author{A.~Lozar}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 12423
  \author{T.~Lueck}\affiliation{\instLMU} % 2406
% \author{T.~Luo}\affiliation{\instFudan} % 3268
  \author{C.~Lyu}\affiliation{\instBonn} % 12484
  \author{Y.~Ma}\affiliation{\instRIKENMSL} % 16883
% \author{A.~Maeda}\affiliation{\instNagoya} % 14664
  \author{M.~Maggiora}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 5343
  \author{S.~P.~Maharana}\affiliation{\instIITHyderabad} % 19083
% \author{T.~Mahood}\affiliation{\instHawaii} % 26003
  \author{R.~Maiti}\affiliation{\instTorinoINFN} % 12043
% \author{S.~Maity}\affiliation{\instIITBhubaneswar} % 2985
  \author{G.~Mancinelli}\affiliation{\instCPPM} % 20743
  \author{R.~Manfredi}\affiliation{\instBNL} % 10303
  \author{E.~Manoni}\affiliation{\instPerugiaINFN} % 2305
% \author{A.~C.~Manthei}\affiliation{\instBonn} % 15023
  \author{M.~Mantovano}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 19783
  \author{D.~Marcantonio}\affiliation{\instMelbourne} % 11163
  \author{S.~Marcello}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 4223
  \author{C.~Marinas}\affiliation{\instIFIC} % 2133
  \author{C.~Martellini}\affiliation{\instRomaTreINFN} % 16983
  \author{A.~Martens}\affiliation{\instIJCLab} % 13823
% \author{A.~Martini}\affiliation{\instDESY} % 2336
  \author{T.~Martinov}\affiliation{\instDESY} % 19463
  \author{L.~Massaccesi}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 16323
  \author{M.~Masuda}\affiliation{\instRCNP}\affiliation{\instEri} % 2238
% \author{T.~Matsuda}\affiliation{\instUOM} % 5543
% \author{K.~Matsuoka}\affiliation{\instKEK}\affiliation{\instNagoya} % 2316
  \author{D.~Matvienko}\affiliation{\instBINP}\affiliation{\instNSU} % 2351
  \author{S.~K.~Maurya}\affiliation{\instIITGuwahati} % 9763
  \author{M.~Maushart}\affiliation{\instIPHC} % 21203
% \author{F.~Mawas}\affiliation{\instIJCLab} % 20943
  \author{J.~A.~McKenna}\affiliation{\instUBC} % 2392
  \author{Z.~Mediankin~Gruberov\'{a}}\affiliation{\instPrague} % 8824
% \author{F.~Meggendorfer}\affiliation{\instMPP} % 7103
  \author{R.~Mehta}\affiliation{\instTata} % 15203
  \author{F.~Meier}\affiliation{\instDuke} % 3103
  \author{D.~Meleshko}\affiliation{\instGiessen} % 11523
  \author{M.~Merola}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2456
% \author{F.~Metzner}\affiliation{\instBonn} % 2296
% \author{M.~Milesi}\affiliation{\instMelbourne} % 5443
  \author{C.~Miller}\affiliation{\instVictoria} % 2273
  \author{M.~Mirra}\affiliation{\instNapoliINFN} % 14744
  \author{S.~Mitra}\affiliation{\instISU} % 19944
  \author{K.~Miyabayashi}\affiliation{\instNaraWu}\affiliation{\instKEK} % 2327
% \author{H.~Miyake}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2452
% \author{R.~Mizuk}\affiliation{\instIJCLab} % 2483
  \author{G.~B.~Mohanty}\affiliation{\instTata} % 2278
  \author{S.~Mondal}\affiliation{\instTorinoINFN} % 19743
  \author{S.~Moneta}\affiliation{\instPerugiaINFN} % 13303
% \author{H.~Moon}\affiliation{\instKoreaUnivKU} % 2304
  \author{A.~L.~Moreira~de~Carvalho}\affiliation{\instDESY} % 26403
  \author{H.-G.~Moser}\affiliation{\instMPP} % 2120
% \author{M.~Mrvar}\affiliation{\instHEPHYVienna} % 2527
% \author{Th.~Muller}\affiliation{\instKarlsruhe} % 2165
  \author{R.~Mussa}\affiliation{\instTorinoINFN} % 2372
  \author{I.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 3463
% \author{K.~R.~Nakamura}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2417
% \author{E.~Nakano}\affiliation{\instOsakaMetropolitan} % 2554
% \author{T.~Nakano}\affiliation{\instRCNP} % 2983
  \author{M.~Nakao}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2498
% \author{H.~Nakayama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2232
% \author{H.~Nakazawa}\affiliation{\instNTUTaiwan} % 2335
  \author{Y.~Nakazawa}\affiliation{\instKEK} % 17383
% \author{A.~Narimani~Charan}\affiliation{\instDESY} % 10143
  \author{M.~Naruki}\affiliation{\instKyotoU} % 4583
  \author{Z.~Natkaniec}\affiliation{\instKrakow} % 3923
  \author{A.~Natochii}\affiliation{\instBNL} % 12063
% \author{L.~Nayak}\affiliation{\instIITHyderabad} % 9464
  \author{M.~Nayak}\affiliation{\instIISc} % 2371
% \author{G.~Nazaryan}\affiliation{\instYerevan} % 9523
  \author{M.~Neu}\affiliation{\instKarlsruhe} % 23304
% \author{C.~Niebuhr}\affiliation{\instDESY} % 2477
% \author{M.~Niiyama}\affiliation{\instKSU} % 2063
% \author{J.~Ninkovic}\affiliation{\instMPGHLL} % 2386
  \author{S.~Nishida}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instNiigata} % 2571
% \author{K.~Nishimura}\affiliation{\instHawaii} % 3063
% \author{A.~Novosel}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 15523
% \author{S.~Ogawa}\affiliation{\instToho} % 6263
  \author{R.~Okubo}\affiliation{\instNagoya} % 10743
% \author{S.~L.~Olsen}\affiliation{\instCAU} % 4563
  \author{H.~Ono}\affiliation{\instNiigata} % 2160
  \author{Y.~Onuki}\affiliation{\instUTokyo} % 2331
% \author{P.~Oskin}\affiliation{\instIJCLab} % 9623
% \author{F.~Otani}\affiliation{\instUTokyo} % 16244
  \author{E.~R.~Oxford}\affiliation{\instCMU} % 6943
% \author{H.~Ozaki}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2984
% \author{P.~Pakhlov}\affiliation{\instHSE} % 2221
  \author{G.~Pakhlova}\affiliation{\instHSE} % 2188
% \author{A.~Panta}\affiliation{\instMississippi} % 7943
% \author{E.~Paoloni}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2488
  \author{S.~Pardi}\affiliation{\instNapoliINFN} % 2532
  \author{K.~Parham}\affiliation{\instDuke} % 10684
  \author{H.~Park}\affiliation{\instKyungpook} % 2284
  \author{J.~Park}\affiliation{\instUTokyo} % 18203
% \author{K.~Park}\affiliation{\instKISTI} % 12243
  \author{S.-H.~Park}\affiliation{\instKEK} % 2509
  \author{B.~Paschen}\affiliation{\instBonn} % 2159
  \author{A.~Passeri}\affiliation{\instRomaTreINFN} % 2116
  \author{S.~Patra}\affiliation{\instLouisville} % 3123
  \author{S.~Paul}\affiliation{\instTUM} % 2131
  \author{T.~K.~Pedlar}\affiliation{\instLuther} % 2421
  \author{I.~Peruzzi}\affiliation{\instFrascati} % 2253
% \author{R.~Peschke}\affiliation{\instHawaii} % 7123
  \author{R.~Pestotnik}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2476
% \author{F.~Pham}\affiliation{\instMelbourne} % 2963
% \author{M.~Piccolo}\affiliation{\instFrascati} % 2147
  \author{L.~E.~Piilonen}\affiliation{\instVPI} % 2346
  \author{P.~L.~M.~Podesta-Lerma}\affiliation{\instUAS} % 2266
  \author{T.~Podobnik}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 11223
% \author{S.~Pokharel}\affiliation{\instMississippi} % 12283
% \author{V.~Popov}\affiliation{\instTelAviv}\affiliation{\instHSE} % 2096
  \author{A.~Prakash}\affiliation{\instLMU} % 21663
  \author{C.~Praz}\affiliation{\instKEK} % 2726
  \author{S.~Prell}\affiliation{\instISU} % 12743
  \author{E.~Prencipe}\affiliation{\instGiessen} % 2219
  \author{M.~T.~Prim}\affiliation{\instBonn} % 2501
  \author{S.~Privalov}\affiliation{\instBINP}\affiliation{\instNSU} % 12503
% \author{I.~Prudiiev}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 19383
% \author{M.~V.~Purohit}\affiliation{\instSCarolina} % 2196
  \author{H.~Purwar}\affiliation{\instHawaii} % 12363
% \author{N.~Rad}\affiliation{\instDESY} % 11683
  \author{P.~Rados}\affiliation{\instNagoya} % 7383
  \author{G.~Raeuber}\affiliation{\instHEPHYVienna} % 18143
  \author{S.~Raiz}\affiliation{\instDESY} % 13003
  \author{V.~Raj}\affiliation{\instIITMadras} % 24983
% \author{N.~Rauls}\affiliation{\instGoettingen} % 11603
  \author{K.~Ravindran}\affiliation{\instTata} % 22503
  \author{J.~U.~Rehman}\affiliation{\instKrakow} % 19623
  \author{M.~Reif}\affiliation{\instMPP} % 8043
  \author{S.~Reiter}\affiliation{\instGiessen} % 2248
  \author{M.~Remnev}\affiliation{\instBINP}\affiliation{\instNSU} % 2785
  \author{L.~Reuter}\affiliation{\instKarlsruhe} % 16403
  \author{D.~Ricalde~Herrmann}\affiliation{\instTabuk} % 9263
  \author{I.~Ripp-Baudot}\affiliation{\instIPHC} % 2469
% \author{M.~Ritzert}\affiliation{\instHeidelberg} % 2526
  \author{G.~Rizzo}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2579
% \author{L.~B.~Rizzuto}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 3746
  \author{S.~H.~Robertson}\affiliation{\instUofA}\affiliation{\instIPP} % 2471
% \author{P.~Rocchetti}\affiliation{\instMelbourne} % 13763
% \author{D.~Rodr\'{i}guez~P\'{e}rez}\affiliation{\instUAS} % 2176
% \author{M.~Roehrken}\affiliation{\instDESY} % 11883
  \author{J.~M.~Roney}\affiliation{\instVictoria}\affiliation{\instIPP} % 2244
% \author{C.~Rosenfeld}\affiliation{\instSCarolina} % 2082
  \author{A.~Rostomyan}\affiliation{\instDESY} % 2481
  \author{N.~Rout}\affiliation{\instDESY} % 2965
% \author{M.~Rozanska}\affiliation{\instKrakow} % 2205
% \author{G.~Russo}\affiliation{\instNapoliUNIV}\affiliation{\instNapoliINFN} % 2388
% \author{D.~Sahoo}\affiliation{\instISU} % 2110
% \author{Y.~Sakai}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2175
% \author{L.~Salutari}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 17423
% \author{G.~Sanchez}\affiliation{\instUNAM} % 2943
  \author{D.~A.~Sanders}\affiliation{\instMississippi} % 2458
  \author{S.~Sandilya}\affiliation{\instIITHyderabad} % 2286
% \author{A.~Sangal}\affiliation{\instCincinnati} % 2384
  \author{L.~Santelj}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2185
  \author{C.~Santos}\affiliation{\instIPHC} % 23743
% \author{Y.~Sato}\affiliation{\instKEK} % 5243
  \author{V.~Savinov}\affiliation{\instPittsburgh} % 2292
  \author{B.~Scavino}\affiliation{\instUppsala} % 2518
  \author{C.~Schmitt}\affiliation{\instLMU}\affiliation{\instMPP} % 15063
% \author{J.~Schmitz}\affiliation{\instBonn} % 12863
% \author{S.~Schneider}\affiliation{\instDuke} % 16803
  \author{M.~Schnepf}\affiliation{\instKarlsruhe} % 15683
  \author{K.~Schoenning}\affiliation{\instUppsala} % 22023
% \author{J.~Schueler}\affiliation{\instHawaii} % 2824
  \author{C.~Schwanda}\affiliation{\instHEPHYVienna} % 2108
  \author{A.~J.~Schwartz}\affiliation{\instCincinnati} % 2162
% \author{B.~Schwenker}\affiliation{\instGoettingen} % 2405
% \author{M.~Schwickardi}\affiliation{\instGoettingen} % 14743
  \author{Y.~Seino}\affiliation{\instNiigata} % 2517
  \author{A.~Selce}\affiliation{\instRomaTreINFN} % 9043
  \author{K.~Senyo}\affiliation{\instYamagata} % 2987
  \author{J.~Serrano}\affiliation{\instCPPM} % 12124
  \author{M.~E.~Sevior}\affiliation{\instMelbourne} % 2328
  \author{C.~Sfienti}\affiliation{\instMainz} % 2214
  \author{W.~Shan}\affiliation{\instHUNNU} % 11943
% \author{C.~Sharma}\affiliation{\instMNITJaipur} % 11584
  \author{G.~Sharma}\affiliation{\instIITMadras} % 18423
% \author{V.~Shebalin}\affiliation{\instHawaii} % 2339
% \author{C.~P.~Shen}\affiliation{\instFudan}\affiliation{\instZZU} % 2464
  \author{X.~D.~Shi}\affiliation{\instUTokyo} % 18843
% \author{H.~Shibuya}\affiliation{\instToho} % 2234
  \author{T.~Shillington}\affiliation{\instMcGill} % 7983
  \author{T.~Shimasaki}\affiliation{\instUTokyo} % 16263
% \author{M.~Shimomura}\affiliation{\instNaraWu} % 2112
  \author{J.-G.~Shiu}\affiliation{\instNTUTaiwan} % 2412
  \author{D.~Shtol}\affiliation{\instBINP}\affiliation{\instNSU} % 9223
  \author{B.~Shwartz}\affiliation{\instBINP}\affiliation{\instNSU} % 2122
  \author{A.~Sibidanov}\affiliation{\instHawaii} % 2419
  \author{F.~Simon}\affiliation{\instKarlsruhe} % 2164
% \author{J.~B.~Singh}\affiliation{\instPanjab}\affiliation{\instUPES} % 2903
  \author{J.~Skorupa}\affiliation{\instMPP}\affiliation{\instTUM} % 12523
% \author{K.~Smith}\affiliation{\instMelbourne} % 2243
  \author{R.~J.~Sobie}\affiliation{\instVictoria}\affiliation{\instIPP} % 2472
  \author{M.~Sobotzik}\affiliation{\instMainz} % 8604
  \author{A.~Soffer}\affiliation{\instTelAviv} % 2217
  \author{A.~Sokolov}\affiliation{\instIHEPRussia} % 2521
% \author{Y.~Soloviev}\affiliation{\instDESY} % 2479
  \author{E.~Solovieva}\affiliation{\instBINP} % 2398
% \author{W.~Song}\affiliation{\instJLU} % 22863
  \author{S.~Spataro}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 2117
  \author{B.~Spruck}\affiliation{\instMainz} % 2493
% \author{S.~Stani\v{c}}\affiliation{\instNovaGorica} % 3383
  \author{M.~Stari\v{c}}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2326
  \author{P.~Stavroulakis}\affiliation{\instIPHC} % 20643
  \author{S.~Stefkova}\affiliation{\instBonn} % 8783
  \author{L.~Stoetzer}\affiliation{\instHawaii} % 19283
% \author{Z.~S.~Stottler}\affiliation{\instVPI} % 2267
  \author{R.~Stroili}\affiliation{\instPadovaUNIV}\affiliation{\instPadovaINFN} % 2465
% \author{J.~Strube}\affiliation{\instPNNL} % 2451
% \author{J.~Su}\affiliation{\instNTUTaiwan} % 16623
% \author{Y.~Sue}\affiliation{\instNagoya} % 2085
% \author{R.~Sugiura}\affiliation{\instUTokyo} % 4644
  \author{M.~Sumihama}\affiliation{\instRCNP}\affiliation{\instGifu} % 4243
% \author{K.~Sumisawa}\affiliation{\instKEK}\affiliation{\instSOKENDAI}\affiliation{\instNaraWu} % 2583
% \author{W.~Sutcliffe}\affiliation{\instBonn} % 3784
% \author{N.~Suwonjandee}\affiliation{\instChula} % 14063
  \author{H.~Svidras}\affiliation{\instDESY} % 11783
% \author{M.~Takahashi}\affiliation{\instDESY} % 2467
  \author{M.~Takizawa}\affiliation{\instSPU}\affiliation{\instJPARC}\affiliation{\instRIKENMSL} % 2437
% \author{U.~Tamponi}\affiliation{\instTorinoINFN} % 2366
% \author{S.~Tanaka}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2530
  \author{S.~S.~Tang}\affiliation{\instFudan} % 12003
  \author{K.~Tanida}\affiliation{\instJAEA} % 3803
% \author{H.~Tanigawa}\affiliation{\instUTokyo} % 2237
% \author{N.~Taniguchi}\affiliation{\instKEK} % 2285
  \author{F.~Tenchini}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 2546
  \author{F.~Testa}\affiliation{\instTorinoUNIV}\affiliation{\instTorinoINFN} % 14844
% \author{A.~Thaller}\affiliation{\instCPPM} % 16044
  \author{O.~Tittel}\affiliation{\instMPP} % 8663
  \author{R.~Tiwary}\affiliation{\instTYL} % 10403
  \author{D.~Tonelli}\affiliation{\instTriesteINFN} % 4564
  \author{E.~Torassa}\affiliation{\instPadovaINFN} % 2556
% \author{N.~Toutounji}\affiliation{\instSydney} % 2263
  \author{K.~Trabelsi}\affiliation{\instTYL} % 2369
  \author{F.~F.~Trantou}\affiliation{\instPisaUNIV}\affiliation{\instPisaINFN} % 23643
  \author{I.~Tsaklidis}\affiliation{\instBonn} % 13443
% \author{T.~Tsuboyama}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2361
% \author{N.~Tsuzuki}\affiliation{\instNagoya} % 2352
  \author{M.~Uchida}\affiliation{\instTitech} % 2370
  \author{I.~Ueda}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2519
% \author{S.~Uehara}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2586
% \author{Y.~Uematsu}\affiliation{\instUTokyo} % 5883
% \author{E.~Uenlue}\affiliation{\instLMU} % 22283
  \author{T.~Uglov}\affiliation{\instHSE} % 2252
  \author{K.~Unger}\affiliation{\instKarlsruhe} % 9463
  \author{Y.~Unno}\affiliation{\instHanyang} % 2420
  \author{K.~Uno}\affiliation{\instKEK} % 14963
  \author{S.~Uno}\affiliation{\instKEK}\affiliation{\instSOKENDAI} % 2149
  \author{P.~Urquijo}\affiliation{\instMelbourne} % 2302
  \author{Y.~Ushiroda}\affiliation{\instKEK}\affiliation{\instUTokyo}\affiliation{\instSOKENDAI} % 2317
% \author{Y.~V.~Usov}\affiliation{\instBINP}\affiliation{\instNSU} % 5003
  \author{S.~E.~Vahsen}\affiliation{\instHawaii} % 2251
  \author{R.~van~Tonder}\affiliation{\instKarlsruhe} % 2706
  \author{K.~E.~Varvell}\affiliation{\instSydney} % 2545
  \author{M.~Veronesi}\affiliation{\instISU} % 20723
% \author{A.~Vinokurova}\affiliation{\instBINP}\affiliation{\instNSU} % 2289
  \author{V.~S.~Vismaya}\affiliation{\instIITHyderabad} % 16063
  \author{L.~Vitale}\affiliation{\instTriesteUNIV}\affiliation{\instTriesteINFN} % 2415
% \author{V.~Vobbilisetti}\affiliation{\instIFIC} % 7364
  \author{R.~Volpe}\affiliation{\instPrague} % 20183
% \author{A.~Vossen}\affiliation{\instDuke} % 2249
% \author{B.~Wach}\affiliation{\instMPP}\affiliation{\instTUM} % 8203
% \author{E.~Waheed}\affiliation{\instMelbourne} % 2226
  \author{M.~Wakai}\affiliation{\instUBC} % 3583
% \author{H.~M.~Wakeling}\affiliation{\instMcGill} % 3664
  \author{S.~Wallner}\affiliation{\instMPP} % 20363
% \author{W.~Wan~Abdullah}\affiliation{\instMalaya} % 2280
% \author{B.~Wang}\affiliation{\instCincinnati} % 2569
% \author{E.~Wang}\affiliation{\instPittsburgh} % 10983
% \author{L.~Wang}\affiliation{\instShandong} % 22443
  \author{M.-Z.~Wang}\affiliation{\instNTUTaiwan} % 2074
  \author{X.~L.~Wang}\affiliation{\instFudan} % 2076
% \author{Z.~Wang}\affiliation{\instUTokyo} % 15743
  \author{A.~Warburton}\affiliation{\instMcGill} % 2347
% \author{M.~Watanabe}\affiliation{\instNiigata} % 2309
  \author{S.~Watanuki}\affiliation{\instCincinnati} % 6843
% \author{M.~Welsch}\affiliation{\instBonn} % 7023
% \author{O.~Werbycka}\affiliation{\instTriesteINFN} % 6123
  \author{C.~Wessel}\affiliation{\instDESY} % 2100
% \author{J.~Wiechczynski}\affiliation{\instKrakow} % 2604
  \author{E.~Won}\affiliation{\instKoreaUnivKU} % 2410
% \author{L.~J.~Wu}\affiliation{\instHNU} % 2704
% \author{Y.~Xie}\affiliation{\instShandong} % 20383
% \author{X.~P.~Xu}\affiliation{\instSoochow} % 4923
% \author{Z.~Xu}\affiliation{\instUTokyo} % 27103
  \author{B.~D.~Yabsley}\affiliation{\instSydney} % 3645
  \author{S.~Yamada}\affiliation{\instKEK} % 2492
  \author{W.~Yan}\affiliation{\instUSTC} % 2094
% \author{W.~C.~Yan}\affiliation{\instZZU} % 2183
  \author{S.~B.~Yang}\affiliation{\instKoreaUnivKU} % 2374
  \author{J.~Yelton}\affiliation{\instFlorida} % 2067
  \author{K.~Yi}\affiliation{\instNNU} % 12583
  \author{J.~H.~Yin}\affiliation{\instNankai} % 2365
% \author{Y.~M.~Yook}\affiliation{\instIHEPChina} % 2453
  \author{K.~Yoshihara}\affiliation{\instHawaii} % 12663
% \author{B.~Yu}\affiliation{\instLMU} % 15563
% \author{C.~Z.~Yuan}\affiliation{\instIHEPChina} % 2088
  \author{J.~Yuan}\affiliation{\instJLU} % 23423
  \author{Y.~Yusa}\affiliation{\instNiigata} % 2357
  \author{L.~Zani}\affiliation{\instRomaTreUNIV}\affiliation{\instRomaTreINFN} % 2529
  \author{F.~Zeng}\affiliation{\instIPMU} % 22043
  \author{M.~Zeyrek}\affiliation{\instMETU} % 4023
  \author{B.~Zhang}\affiliation{\instHawaii} % 11663
% \author{J.~Z.~Zhang}\affiliation{\instIHEPChina} % 2349
% \author{Y.~Zhang}\affiliation{\instFudan} % 3303
% \author{Z.~Zhang}\affiliation{\instUSTC} % 5363
% \author{J.~Zhao}\affiliation{\instIHEPChina} % 3343
  \author{V.~Zhilich}\affiliation{\instBINP}\affiliation{\instNSU} % 4703
  \author{J.~S.~Zhou}\affiliation{\instFudan} % 12463
  \author{Q.~D.~Zhou}\affiliation{\instShandong} % 7323
% \author{X.~Y.~Zhou}\affiliation{\instLNNU} % 2380
  \author{L.~Zhu}\affiliation{\instJLU} % 25143
% \author{V.~I.~Zhukova}\affiliation{\instLjubljanaUniLJ}\affiliation{\instLjubljanaJSI} % 2387
% \author{V.~Zhulanov}\affiliation{\instBINP}\affiliation{\instNSU} % 4983
  \author{R.~\v{Z}leb\v{c}\'{i}k}\affiliation{\instTriesteINFN} % 13403
% \author{S.~Zou}\affiliation{\instFudan} % 19363
\collaboration{The Belle II Collaboration}

